Integral of Map into Abelian $\Omega$-group

The common in ring, module and algebra is that they are Abelian group with respect to addition. This property is enough to study integration. I treat integral of measurable map into normed Abelian $\Omega$-group. Theory of integration of maps into $\Omega$-group has a lot of common with theory of integration of functions of real variable. However I had to change some statements, since they implicitly assume either compactness of range or total order in $\Omega$-group.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau I}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, механика,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 3}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $3$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{1310.5591}
{
Александр Клейн,
Интеграл отображения в абелевую $\Omega$\Hyph группу,\\
eprint \href{http://arxiv.org/abs/1310.5591}{arXiv:1310.5591} (2013)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Aleks Kleyn.\\
Linear Algebra over Division Ring: System of Linear Equations.\\
Create Space, 2012; ISBN-13: 978-1477631812
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fikhtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Fikhtengolts: Calculus volume 3}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 3,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper,1211.6965,4910-5816,GJSFRF.Basis,1302.7204,CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,1211.6965,4910-5816,CACAA.01.195,GJSFRF.Basis,1302.7204}
\Items{CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis,1302.7204,CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
Очень трудно провести границу между модулем и алгеброй.
Тем более, иногда в процессе построения мы должны сперва
доказать, что множество $A$ является модулем,
а потом мы доказываем, что это множество является алгеброй.
Поэтому для записи координат элемента модуля
мы также будем пользоваться соглашением
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{1302.7204,CACAA.02.97,1310.5591,MSimplex,MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
\ePrints{1302.7204,CACAA.02.97,MSimplex}
\ifx\Semafor\ValueOn
$D$\Hyph алгебры
\else
$\Omega$\Hyph группы
\fi
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph число, а кватернион называется $H$\Hyph число.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763}
\ifx\Semafor\ValueOn
\begin{convention}
Отождествление вектора и матрицы его координат
может привести к неоднозначности в равенстве
\ShowEq{Identification can lead to ambiguity, 1}
где $\Basis e$ - базис векторного пространства.
Поэтому мы будем записывать равенство
\EqRef{Identification can lead to ambiguity, 1}
в виде
\ShowEq{Identification can lead to ambiguity, 2}
чтобы видеть, где записан вектор.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.01.195}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,1305.4547,1310.5591}
\Items{1003.3714,4820-2669,MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ePrints{MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Мы будем полагать,
что рассматриваемая мера является полной мерой.
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Fubini.Russian.tex <==
%auto-ignore
\input{Fubini.Eq}
\ifx\PrintBook\Defined
\chapter{Теорема Фубини}
\fi

\section{Произведение полуколец множеств}

\begin{definition}
Пусть
\ShowEq{L1n}
- система подмножеств множества \(A_i\).
\AddIndex{Декартово произведение систем подмножеств}
{Cartesian product of systems of subsets}
\ShowEq{Cartesian product of systems of subsets}
является системой подмножеств множества
\ShowEq{A=xA1n},
представимых в виде\footnote{Смотри также определение в
\citeBib{Kolmogorov Fomin} на странице 310.}
\ShowEq{C=xC1n}
Если
\ShowEq{Li=L}
то система множеств
\ShowEq{Cartesian power of systems of subsets}
называется
\AddIndex{декартова степень \(n\) систем подмножеств}
{Cartesian power of systems of subsets}
\qed
\end{definition}

\begin{theorem}
Декартово произведение\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 311.}
\ShowEq{S1x...xSn}
полуколец множеств
\ShowEq{semirings S1n}
является полукольцом множеств.
\end{theorem}
\begin{proof}
Мы докажем теорему для случая \(n=2\).
В общем случае доказательство аналогично.

\StartLabelItem
\begin{enumerate}
\item
Пусть
\ShowEq{A B in S12}
Следовательно
\ShowEq{A=A1xA2}
\ShowEq{B=B1xB2}
Очевидно, что
\ShowEq{x in A*B}
тогда и только тогда, когда
\ShowEq{x in A*B 12}
Следовательно
\ShowEq{A*B=A*B 12}
Из
\EqRef{A=A1xA2},
\EqRef{B=B1xB2}
и утверждения
\RefItem{AB in S}
следует, что
\ShowEq{AB12 in S}
Из
\EqRef{A=A1xA2},
\EqRef{B=B1xB2},
\EqRef{AB12 in S}
следует, что
\ShowEq{AB 12 in S}
Следовательно, утверждение
\RefItem{AB in S}
верно для
\ShowEq{S1xS2}.
\LabelItem{AB in S1xS2}
\item
Пусть
\ShowEq{Bi in Ai}
Из утверждения
\RefItem{A=+Ai}
следует, что
\ShowEq{A1=B1+}
\ShowEq{A2=B2+}
Из
\EqRef{A1=B1+},
\EqRef{A2=B2+}
следует, что
\ShowEq{x in A1xA2}
тогда и только тогда, когда
\((x_1,x_2)\)
принадлежит одному из следующих множеств:
\ShowEq{BixBj}
Следовательно,
\ShowEq{Ax=Bx+}
и утверждение
\RefItem{A=+Ai}
верно для
\ShowEq{S1xS2}.
\LabelItem{A=+Ai, S1xS2}
\end{enumerate}

Из рассуждений
\RefItem{AB in S1xS2},
\RefItem{A=+Ai, S1xS2}
следует, что
\ShowEq{S1xS2}
является полукольцом множеств.
\end{proof}

Однако декартово произведение колец множеств,
вообще говоря, не является кольцом множеств.

\begin{definition}
Кольцо множеств
\ShowEq{product of rings of sets}
порождённое полукольцом множеств
\ShowEq{R1x...xRn}
называется
\AddIndex{произведением колец множеств}{product of rings of sets}
\ShowEq{R1n}
\qed
\end{definition}

\begin{theorem}
Произведение алгебр множеств является алгеброй множеств.
\end{theorem}
\begin{proof}
Для
\ShowEq{i1n},
пусть кольцо множеств \(\mathcal R_i\)
является алгеброй множеств.
Согласно определению
\ref{definition: algebra of sets},
алгебра множеств \(\mathcal R_i\)
имеет единицу \(E_i\) такую, что
\ShowEq{Ai*Ei=Ai}
для любого
\ShowEq{Ai in Ri}
Из рассуждения
\RefItem{AB in S1xS2}
и из
\EqRef{Ai*Ei=Ai}
следует, что
\ShowEq{xAi*xEi=xAi}
Из теоремы
\ref{theorem: ring of sets generated by semiring}
и равенства
\EqRef{xAi*xEi=xAi}
следует, что
для любого
\ShowEq{A in xR}
верно равенство
\ShowEq{A*xEi=A}
Следовательно, множество
\ShowEq{xEi}
является единицей кольца множеств
\ShowEq{xRi}.
Согласно определению
\ref{definition: algebra of sets},
кольцо множеств
\ShowEq{xRi}
является алгеброй множеств.
\end{proof}

\section{Произведение мер}

\begin{theorem}
\label{theorem: Cartesian product of measures}
Пусть
\ShowEq{mui:Ri->R}
мера на полукольце
\ShowEq{Ri 1n}
\AddIndex{Декартово произведение}{Cartesian product of measures}
\ShowEq{Cartesian product of measures}
{\bf мер}
определено формулой\footnote{Смотри
\citeBib{Kolmogorov Fomin}, страница 312,
доказательство, что отображение, определённое формулой
\EqRef{muA1n=*muAi},
является мерой.
}
\ShowEq{muA1n=*muAi}
\end{theorem}
\begin{proof}
Мы докажем теорему для случая \(n=2\).
В общем случае доказательство аналогично.
Пусть
\ShowEq{A1xA2=+Bi}
где
\ShowEq{Bi*Bj=empty}
и
\ShowEq{Bi=Bi1xBi2}
Согласно лемме
\ref{lemma: exists finite expansion of set, 2},
существуют разложения
\ShowEq{Ai=+Cim}
такие, что
\ShowEq{Bik=+Cim}
\ShowEq{M1k M2k}
Согласно утверждению
\RefItem{m A=+m Ai}
по отношению к мерам
\ShowEq{mu12}
из
%\EqRef{A1xA2=+Bi},
\EqRef{Bik=+Cim}
следует, что
\ShowEq{muA=+muBk}
Из
\EqRef{A1xA2=+Bi},
\EqRef{muA=+muBk}
следует, что утверждение
\RefItem{m A=+m Ai}
верно для \(\mu\).
\end{proof}

\begin{theorem}
Пусть
\ShowEq{mui 1n}
- \(\sigma\)\Hyph аддитивная мера,\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 2 на странице 313.}
определённая на \(\sigma\)\Hyph алгебре \(\mathcal C_i\).
Декартово произведение мер
\ShowEq{mu1x...xmun}
является \(\sigma\)\Hyph аддитивной мерой на полукольце
\ShowEq{C1x...xCn}
\end{theorem}
\begin{proof}
Мы докажем теорему для случая \(n=2\).
В общем случае доказательство аналогично.
Пусть
\ShowEq{C=+Cn infty}
где
\ShowEq{Cn*Cm=0}
Согласно
\EqRef{C=+Cn infty}
\ShowEq{C=AxB}

Рассмотрим множество отображений
\ShowEq{fn:X->R}
определённых правилом
\ShowEq{fn(An)=mu(Bn)}
Пусть \(x\in A\).
Пусть
\ShowEq{Nx=()}
Согласно
\EqRef{Cn*Cm=0},
для любого \(y\in B\)
существует единственное \(n\in N_x\)
такое, что
\ShowEq{xy in ABn}
При этом
\ShowEq{n ne m=>Bn*Bm=0}
Согласно утверждению
\RefItem{mu(X=+Xi)}
относительно меры \(\mu_2\)
\ShowEq{+fn(x)=mu2(B)}
Согласно теоремам
\ref{theorem: int f+g X},
\ref{theorem: int ag=a int g}
и следствию
\ref{corollary: int X f(x)=lim},
равенство
\ShowEq{+int fn(x)}
является следствием равенства
\EqRef{+fn(x)=mu2(B)}.
Согласно теореме
\ref{theorem: int ag=a int g},
равенство
\ShowEq{int fn(x)}
является следствием равенства
\EqRef{fn(An)=mu(Bn)}.
Равенство
\ShowEq{mu(C)=+mu(Cn)}
является следствием равенств
\EqRef{+int fn(x)},
\EqRef{int fn(x)}.
Следовательно, утверждение
\RefItem{mu(X=+Xi)}
верно для меры \(\mu\).
\end{proof}

Лебегово
продолжение меры
\ShowEq{mu1x...xmun}
определённое на \(\sigma\)\Hyph алгебре
\ShowEq{C supset C1x...xCn},
называется
\AddIndex{произведением мер}{product of measures}
\ShowEq{product of measures}
Если
\ShowEq{mu1=...=mun}
то произведение мер называется
\AddIndex{степенью меры}{power of measure} \(\mu\)
\ShowEq{power of measure}

\begin{theorem}
\label{theorem: evaluation of product measure}
Пусть
\ShowEq{mui 12}
- \(\sigma\)\Hyph аддитивная мера,\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 3 на странице 314.
Я не предполагаю, что \(X_i\) - множество действительных чисел.}
определённая на \(\sigma\)\Hyph алгебре \(\mathcal C_i\)
подмножеств множества \(X_i\).
Пусть
\ShowEq{mu=mu1mu2}
Пусть
\ShowEq{A in C1C2}

Пусть для каждого \(x_1\in X_1\)
\ShowEq{Ax1=()}
Если отображение
\ShowEq{x1->Ax1}
\(\mu_1\)\Hyph интегрируемо, то
\EquationParm{mu(A)=int dmu1 mu2}{A a=1 b=2}

Пусть для каждого \(x_2\in X_2\)
\ShowEq{Ax2=()}
Если отображение
\ShowEq{x2->Ax2}
\(\mu_2\)\Hyph интегрируемо, то
\EquationParm{mu(A)=int dmu1 mu2}{A a=2 b=1}
\end{theorem}
\begin{proof}
Мы докажем равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}.
Доказательство равенства
\EqRefParm{mu(A)=int dmu1 mu2}{A a=2 b=1}
аналогично.

\begin{lemma}
\label{lemma: mu(A)=int dmu1 mu2, A=A1xA2 0}
Равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}
верно для множества вида
\ShowEq{A=A1xA2 0}
\end{lemma}
{\sc Доказательство.}
Согласно определению
\ref{theorem: Cartesian product of measures},
\ShowEq{mu(A)=mu(A1)mu(A2)}
Согласно
\EqRef{Ax1=()}
\ShowEq{Ax1= A1xA2}
Из
\EqRef{Ax1= A1xA2}
и теоремы
\ref{theorem: m(empty)=0}
следует, что
\ShowEq{mu(Ax1)}
Из
\EqRef{A=A1xA2 0},
\EqRef{mu(Ax1)}
и определения
\ref{definition: simple map}
следует, что
отображение
\ShowEq{x1->mu(Ax1)}
является простым.
Согласно определению
\ref{definition: integrable map},
\ShowEq{int dmu1 mu2 0}
Лемма следует
из равенств
\EqRef{mu(A)=mu(A1)mu(A2)},
\EqRef{int dmu1 mu2 0}.
\hfill\(\odot\)

\begin{lemma}
\label{lemma: mu(A)=int dmu1 mu2, A=A1xA2 1n}
Равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}
верно для множества вида
\ShowEq{A=A1xA2 1n}
\end{lemma}
{\sc Доказательство.}
Согласно лемме
\ref{lemma: exists finite expansion of set, 2},
существует конечная система множеств
\ShowEq{B1j in C}
такая, что
\ShowEq{B1j in C ne}
\ShowEq{A1i=+B1j}
где
\ShowEq{M1i in 1t}
Согласно лемме
\ref{lemma: exists finite expansion of set, 2},
существует конечная система множеств
\ShowEq{B2j in C}
такая, что
\ShowEq{B2j in C ne}
\ShowEq{A2i=+B2j}
где
\ShowEq{M2i in 1t}
Из
\EqRef{B1j in C ne},
\EqRef{B2j in C ne}
следует, что
\ShowEq{*B1ixB2j=0}
Из равенств
\EqRef{A1i=+B1j},
\EqRef{A2i=+B2j}
следует, что для любого \(i\)
\ShowEq{A1ixA2i=+}
Пусть
\ShowEq{Mi=M1ixM2i}
Равенство
\ShowEq{A1ixA2i=+i}
следует из
\EqRef{A1ixA2i=+},
\EqRef{Mi=M1ixM2i}.
Пусть
\ShowEq{M=+Mi}
Равенство
\ShowEq{A=+B1kxB2l}
следует из
\EqRef{A=A1xA2 1n},
\EqRef{A1ixA2i=+i},
\EqRef{M=+Mi}.
Согласно утверждению
\RefItem{m A=+m Ai}
и определению
\ref{theorem: Cartesian product of measures},
\ShowEq{mu(A)=+mu(Ai*)}
следует из
\EqRef{*B1ixB2j=0},
\EqRef{A=+B1kxB2l}.

Согласно
\EqRef{Ax1=()},
\EqRef{A=+B1kxB2l}
\ShowEq{Ax1= A1xA2 1n}
Из равенства
\EqRef{Ax1= A1xA2 1n},
утверждения
\RefItem{m A=+m Ai},
и теоремы
\ref{theorem: m(empty)=0}
следует, что
\ShowEq{mu(Ax1) 1n}
Из
\EqRef{A=+B1kxB2l},
\EqRef{mu(Ax1) 1n}
и определения
\ref{definition: simple map}
следует, что
отображение
\ShowEq{x1->mu(Ax1)}
является простым.
Согласно определению
\ref{definition: integrable map},
\ShowEq{int dmu1 mu2 1n}
Лемма следует
из равенств
\EqRef{mu(A)=+mu(Ai*)},
\EqRef{int dmu1 mu2 1n}.
\hfill\(\odot\)

Согласно теореме
\ref{theorem: A in B, B_1 supseteq B_2, Bn1 subseteq Bn2},
для любого множества
\ShowEq{A in Cmu12}
существует множество \(B\) такое, что
\DrawEq{A in B}{measure product}
\DrawEq{muA=muB}{measure product}
\DrawEq{B=*Bn}{measure product}
\DrawEq{B_1 supseteq B_2}{measure product}
\DrawEq{Bn=+Bnk}{measure product}
\ShowEq{Bnk in Cmu12}
\DrawEq{muBnk<muA+}{measure product}
\DrawEq{Bn1 subseteq Bn2}{measure product}
Согласно леммам
\ref{lemma: mu(A)=int dmu1 mu2, A=A1xA2 0},
\ref{lemma: mu(A)=int dmu1 mu2, A=A1xA2 1n},
из утверждения
\EqRef{Bnk in Cmu12}
следует, что равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}
верно для множеств \(B_{nk}\)
\EquationParm{mu(A)=int dmu1 mu2}{Bnk a=1 b=2}
где
\ShowEq{Bnkx2}
Утверждение
\ShowEq{Bn1x1 subseteq Bn2x1}
является следствием
\eqRef{Bn1 subseteq Bn2}{measure product},
\EqRef{Bnkx2}.
Рассмотрим множество отображений
\ShowEq{fnk:X1->R}
Согласно теореме
\ref{theorem: A in B in Cmu=>mu A<mu B},
утверждение
\ShowEq{fnk<fnk+1}
является следствием утверждения
\EqRef{Bn1x1 subseteq Bn2x1}.
Утверждение
\ShowEq{int fnk<muA+}
является следствием утверждений
\eqRef{muBnk<muA+}{measure product},
\EqRefParm{mu(A)=int dmu1 mu2}{Bnk a=1 b=2}.
Согласно теореме
\ref{theorem: Beppo Levi},
\begin{itemize}
\item
почти всюду на \(X_1\) существует конечный предел
\ShowEq{fn(x)=lim fnk(x)}
\item
отображение \(f_n\) интегрируемо на \(X_1\) и
\ShowEq{int fn=lim int fnk}
\end{itemize}
Утверждение
\ShowEq{lim int fnk=int lim fnk}
является следствием утверждений
\EqRef{fn(x)=lim fnk(x)},
\EqRef{int fn=lim int fnk}.
Утверждение
\ShowEq{Bnx1=+Bnkx1}
где
\DrawEq{Bnx2}{}
следует из цепочки утверждений
\ShowEq{Bnx1=+Bnkx1 1}
Согласно теореме
\ref{theorem: Continuity of sigma-additive measure, subset},
\begin{itemize}
\item
равенства
\ShowEq{lim mu Bnkx1=mu Bnx1}
\ShowEq{lim int fnk=int fn}
являются следствием утверждений
\EqRef{Bn1x1 subseteq Bn2x1},
\EqRef{lim int fnk=int lim fnk},
\EqRef{Bnx1=+Bnkx1}.
\item
равенство
\ShowEq{lim muBnk=muBn}
является следствием утверждений
\eqRef{Bn=+Bnk}{measure product},
\eqRef{Bn1 subseteq Bn2}{measure product}.
\end{itemize}
Из равенств
\EqRefParm{mu(A)=int dmu1 mu2}{Bnk a=1 b=2},
\EqRef{lim int fnk=int fn},
\EqRef{lim muBnk=muBn}
следует, что равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}
верно для множеств \(B_n\)
\EquationParm{mu(A)=int dmu1 mu2}{Bn a=1 b=2}
Утверждение
\ShowEq{B1x1 supseteq B2x1}
является следствием
\eqRef{B_1 supseteq B_2}{measure product},
\EqRef{Bnkx2}.
Равенство
\ShowEq{fn:X1->R}
следует из равенств
\EqRef{fn(x)=lim fnk(x)},
\EqRef{lim mu Bnkx1=mu Bnx1}.
Согласно теореме
\ref{theorem: A in B in Cmu=>mu A<mu B},
утверждение
\ShowEq{fn>fn+1}
является следствием утверждения
\EqRef{B1x1 supseteq B2x1}.
Согласно теореме
\ref{theorem: |int f|<M mu},
утверждение
\ShowEq{int fn>0}
является следствием утверждения
\RefItem{m(A)>0}.
Согласно теореме
\ref{theorem: Beppo Levi},
\begin{itemize}
\item
почти всюду на \(X_1\) существует конечный предел
\ShowEq{f(x1)=lim fn(x1)}
\item
отображение \(f\) интегрируемо на \(X_1\) и
\ShowEq{int f(x1)=lim int fn}
\end{itemize}
Утверждение
\ShowEq{lim int fn=int lim fn}
является следствием утверждений
\EqRef{f(x1)=lim fn(x1)},
\EqRef{int f(x1)=lim int fn}.
Утверждение
\ShowEq{Bx1=*Bnx1}
где
\ShowEq{Bx2=}
следует из цепочки утверждений
\ShowEq{Bx1=*Bnx1 1}
Согласно теореме
\ref{theorem: Continuity of sigma-additive measure, supset},
\begin{itemize}
\item
равенство
\ShowEq{lim int fn=int f}
является следствием утверждений
\EqRef{B1x1 supseteq B2x1},
\EqRef{lim int fn=int lim fn},
\EqRef{Bx1=*Bnx1}.
\item
равенство
\ShowEq{lim muBn=muB}
является следствием утверждений
\eqRef{B=*Bn}{measure product},
\eqRef{B_1 supseteq B_2}{measure product}.
\end{itemize}
Из равенств
\EqRefParm{mu(A)=int dmu1 mu2}{Bn a=1 b=2},
\EqRef{lim int fn=int f},
\EqRef{lim muBn=muB}
следует, что равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}
верно для множества \(B\)
\EquationParm{mu(A)=int dmu1 mu2}{B a=1 b=2}

\begin{lemma}
\label{lemma: muA=0=>int dmu1 mu2=0}
Если
\EquationParm{muA=0}A
то
\EquationParm{int dmu1 mu2=0}A
\end{lemma}
{\sc Доказательство.}
Равенство
\EquationParm{int dmu1 mu2=0}B
следует из равенств
\eqRef{muA=muB}{measure product},
\EqRefParm{muA=0}A.
Согласно теореме
\ref{theorem: int|f|=0=>f=0}
и утверждению
\RefItem{m(A)>0},
равенство
\EquationParm{mu2Bx1=0}B
почти всюду является следствием равенства
\EqRefParm{int dmu1 mu2=0}B.
Утверждение
\ShowEq{Ax1 in Bx1}
является следствием утверждения
\eqRef{A in B}{measure product}.
Согласно теореме
\ref{theorem: A in B, mu B=0},
равенство%
\EquationParm{mu2Bx1=0}A
почти всюду является следствием
\EqRefParm{mu2Bx1=0}B,
\EqRef{Ax1 in Bx1}.
Согласно определению
\ref{definition: integrable map},
равенство
\EqRefParm{int dmu1 mu2=0}A
является следствием равенства
\EqRefParm{mu2Bx1=0}A.
\hfill\(\odot\)

Пусть
\ShowEq{C=B-A}
Тогда
\EquationParm{B=A+C}{no}
\EquationParm{B=A+C}{x1}
Равенства
\ShowEq{muB=muA+muC}
\ShowEq{muB=muA+muC x1}
являются следствием равенств
\EqRefParm{B=A+C}{no},
\EqRefParm{B=A+C}{x1}.
Равенство
\ShowEq{mu(A+C)=int dmu1 mu2}
является следствием равенств
\EqRefParm{mu(A)=int dmu1 mu2}{B a=1 b=2},
\EqRef{muB=muA+muC},
\EqRef{muB=muA+muC x1}
и теоремы
\ref{theorem: int f+g X}.
Равенство
\EquationParm{muA=0}C
является следствием равенств
\eqRef{muA=muB}{measure product},
\EqRef{muB=muA+muC}.
Согласно лемме
\ref{lemma: muA=0=>int dmu1 mu2=0},
равенство
\EquationParm{int dmu1 mu2=0}C
является следствием равенства
\EqRefParm{muA=0}C.
Равенство
\EqRefParm{mu(A)=int dmu1 mu2}{A a=1 b=2}
является следствием равенств
\EqRef{mu(A+C)=int dmu1 mu2},
\EqRefParm{muA=0}C,
\EqRefParm{int dmu1 mu2=0}C.
\end{proof}

\section{Теорема Фубини}

\begin{theorem}[Фубини]
\label{theorem: Fubini}
Пусть \(\mu_1\) и \(\mu_2\) -
\(\sigma\)\Hyph аддитивные полные
меры, определеные на \(\sigma\)\Hyph алгебрах.\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 5 на странице 317.}
Пусть
\ShowEq{mu=mu1mu2}
Пусть \(A\) - полная абелевая \(\Omega\)\Hyph группа.
Пусть отображение
\ShowEq{f:X12->A}
с компактным множеством значений
\(\mu\)\Hyph интегрируемо на множестве
\ShowEq{B in X12}
Тогда
\EquationParm{int B f=int X1 int Bx1 f}{a=1 b=2}
\EquationParm{int B f=int X1 int Bx1 f}{a=2 b=1}
\end{theorem}
\begin{proof}
Мы докажем равенство
\EqRefParm{int B f=int X1 int Bx1 f}{a=1 b=2}.
Доказательство равенства
\EqRefParm{int B f=int X1 int Bx1 f}{a=2 b=1}
аналогично.

\begin{lemma}
\label{lemma: Fubini, simple map}
Равенство
\EqRefParm{int B f=int X1 int Bx1 f}{a=1 b=2}
верно для простого отображения \(f\).
\end{lemma}
{\sc Доказательство.}
Пусть
\ShowEq{range f}
- область значений отображения $f$.
Пусть
\ShowEq{Bi=(f(x12)=yi)}
Так как
\ShowEq{B=+Bi ij=0}
то равенство
\ShowEq{int B f=+muB y}
является следствием определения
\ref{definition: integrable map}.
Равенство
\DrawEqParm{mu(A)=int dmu1 mu2}{Bn a=1 b=2}{Fubini}
где
\DrawEq{Bnx2}{Fubini}
является следствием теоремы
\ref{theorem: evaluation of product measure}.
Равенство
\ShowEq{int B f=+int dmu1 mu2 y}
является следствием равенств
\EqRef{int B f=+muB y},
\eqRefParm{mu(A)=int dmu1 mu2}{Bn a=1 b=2}{Fubini}.
Согласно определению
\ref{definition: integrable map},
равенство
\ShowEq{int Bx1 f=+muBnx1 y}
является следствием равенств
\EqRef{Bi=(f(x12)=yi)},
\eqRef{Bnx2}{Fubini}.
Согласно теоремам
\ref{theorem: int f+g X},
\ref{theorem: int ga=int g a},
равенство
\ShowEq{int X1 int Bx1 f=+int X1 muBnx1 a}
является следствием равенства
\EqRef{int Bx1 f=+muBnx1 y}.
Равенство
\EqRefParm{int B f=int X1 int Bx1 f}{a=1 b=2}
является следствием равенств
\EqRef{int B f=+int dmu1 mu2 y},
\EqRef{int X1 int Bx1 f=+int X1 muBnx1 a}.
\hfill\(\odot\)

Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
существует последовательность
простых  отображений
\ShowEq{fn:X12->A}
сходящаяся равномерно к \(f\)
\DrawEq{f(x)=lim}{Fubini}
Согласно лемме
\ref{lemma: Fubini, simple map},
равенство
\EquationParm{int B f=int X1 int Bx1 f}{fn a=1 b=2}
верно для любого отображения \(f_n\).
Равенства
\EquationParm{int B f=lim}{B x12}
\EquationParm{int B f=lim}{Bx1}
являются следствием определения
\ref{definition: Integral of Map over Set of Finite Measure}.
Так как отображение \(f\)
имеет компактное множество значений,
то существует \(M>0\) такое, что
\ShowEq{|f(x12)|<M}
Согласно построению в доказательстве теоремы
\ref{theorem: uniformly convergent sequence of simple maps},
утверждение
\ShowEq{|fn(x)|<M+1}
являются следствием утверждения
\EqRef{|f(x12)|<M}.
Согласно теореме
\ref{theorem: |int f|<M mu},
утверждение
\ShowEq{|int Bx1 fn|<muBx1(M+1)}
являются следствием утверждения
\EqRef{|fn(x)|<M+1}.
Согласно теоремам
\ref{theorem: int ga=int g a},
\ref{theorem: evaluation of product measure},
отображение
\ShowEq{x1->muBx1()}
\(\mu_1\)\Hyph интегрируемо.
Согласно теореме
\ref{theorem: Lebesgue's bounded convergence theorem},
из
\eqRef{f(x)=lim}{Fubini},
\EqRefParm{int B f=lim}{Bx1}
следует, что отображение
\ShowEq{x1->int Bx1 f}
\(\mu_1\)\Hyph интегрируемо и
\ShowEq{lim int X1 int Bx1 f}
является следствием
\EqRefParm{int B f=lim}{Bx1}.
Равенство
\EqRefParm{int B f=int X1 int Bx1 f}{a=1 b=2}
является следствием равенств
\EqRefParm{int B f=lim}{B x12},
\EqRef{lim int X1 int Bx1 f}.
\end{proof}



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc линейная комбинация
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%789%A%Astar антилинейное отображение алгебры с сопряжением
   {$A\star$\Hyph антилинейное отображение алгебры с сопряжением}%
   {antilinear mapping of algebra with conjugation}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%779%D%Dstar антилинейное отображение кольца с сопряжением
   {$D\star$\Hyph антилинейное отображение кольца с сопряжением}%
   {antilinear mapping of ring with conjugation}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%769%D%Dstar линейный гомоморфизм
   {$D\star$\Hyph линейный гомоморфизм}%
   {Dstar linear homomorphism}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%156%D%Dstar-модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%765%R%RCcircA линейная комбинация
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%192%S%starD- векторное пространство
   {$\star D$\Hyph векторное пространство}%
   {starD vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%832%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%842%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%16%Б%базис drc векторного пространства r строк
   {базис \drc векторного пространства \subs строк}%
   {basis, r rows drc vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%197%Б%базис в D векторном пространстве
   {базис в $D$\Hyph векторном пространстве}%
   {basis, D vector space}%
\Index%24%Б%базис в rcd векторном пространстве
   {базис в \rcd векторном пространстве}%
   {basis, rcd vector space}%
\Index%25%Б%базис в rcd векторном пространстве c строк
   {базис в \rcd векторном пространстве \sups строк}%
   {basis, c rows rcd vector space}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%782%В%вектор отображения
   {вектор отображения}%
   {vector of mapping}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%847%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%849%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%850%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%868%В%внешняя мера
   {внешняя мера}%
   {outer measure}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%829%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%830%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%838%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%848%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%851%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%852%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%845%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%864%Д%декартова степень систем подмножеств
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Index%855%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%863%Д%декартово произведение систем подмножеств
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал Гато отображения
   {дифференциал Гато отображения}%
   {Gateaux differential of map}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%837%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%654%З%закон ассоциативности для D- модуля
   {закон ассоциативности для $D$\Hyph модуля}%
   {associative law, D module}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%501%З%закон ассоциативности для starD- векторного пространства
   {закон ассоциативности для $\star D$\Hyph векторного пространства}%
   {associative law, starD vector space}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%655%З%закон дистрибутивности для D- модуля
   {закон дистрибутивности для $D$\Hyph модуля}%
   {distributive law, D module}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%625%З%закон дистрибутивности для starD- векторного пространства
   {закон дистрибутивности для $\star D$\Hyph векторного пространства}%
   {distributive law, starD vector space}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%656%З%закон унитарности для D- модуля
   {закон унитарности для $D$\Hyph модуля}%
   {unitarity law, D module}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\Index%199%З%закон унитарности для starD- векторного пространства
   {закон унитарности для $\star D$\Hyph векторного пространства}%
   {unitarity law, starD vector space}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%825%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%869%И%измеримое по Лебегу множество
   {измеримое по Лебегу множество}%
   {Lebesgue measurable}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%844%И%интеграл отображения
   {интеграл отображения}%
   {integral of map}%
\Index%843%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%862%К%кольцо множеств, порождённое полукольцом множеств
   {кольцо множеств, порождённое полукольцом множеств}%
   {ring of sets generated by semiring}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%861%К%конечное разложение множества
   {конечное разложение множества}%
   {finite expansion of set}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%859%К%координатное представление вектора
   {координатное представление вектора}%
   {coordinate representation of vector}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%33%Л%Drc линейно независимые векторные поля
   {линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%871%Л%лебегово продолжение меры
   {лебегово продолжение меры}%
   {Lebesgue extension of measure}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear combination of  vectors}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%613%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%398%Л%линейное отображение D векторных пространств
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map of D vector spaces}%
\Index%35%Л%линейное отображение rcd векторных пространств
   {линейное отображение \rcd векторных пространств}%
   {linear map of rcd vector spaces}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%866%М%мера
   {мера}%
   {measure}%
\Index%870%М%мера Лебега
   {мера Лебега}%
   {Lebesgue measure}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%828%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%831%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%835%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%827%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%853%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%860%П%полукольцо множеств
   {полукольцо множеств}%
   {semiring of sets}%
\Index%826%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%834%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%854%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%867%П%продолжение меры
   {продолжение меры}%
   {extension of measure}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%865%П%произведение колец множеств
   {произведение колец множеств}%
   {product of rings of sets}%
\Index%683%П%произведение линейного отображения на скаляр
   {произведение линейного отображения на скаляр}%
   {product of linear map over scalar}%
\Index%856%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%271%П%произведение отображения на скаляр
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%839%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%833%С%связное множество
   {связное множество}%
   {connected set}%
\Index%846%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%836%С%симплекс
   {симплекс}%
   {simplex}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%781%С%скаляр отображения
   {скаляр отображения}%
   {scalar of mapping}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%840%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%841%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%857%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%351%С%сумма линейных отображений
   {сумма линейных отображений}%
   {sum of linear maps}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%207%Т%тензорное произведение векторных пространств
   {тензорное произведение векторных пространств}%
   {tensor product of vector spaces}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%500%Э%эффективное Tstar представление Omega- алгебры A
   {эффективное \Ts представление $\Omega$\Hyph алгебры $A$}%
   {effective Tstar representation of algebra}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%858%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Integral.Russian.tex <==
%auto-ignore
\input{Integral.Eq}
\ifx\PrintBook\Defined
\chapter{Интеграл отображения в абелеву
\texorpdfstring{$\Omega$}{Omega}-группу}
\fi

Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть определено эффективное представление поля действительных чисел \(R\)
в полной абелевой \(\Omega\)\Hyph группе \(A\).\footnote{Другими
словами,
\(\Omega\)\Hyph группа \(A\) является
\(R\)\Hyph векторным пространством.}
В этой главе мы рассмотрим определение
интеграл Лебега
\(\mu\)\Hyph измеримого отображения
\ShowEq{f:X->A}

\section{Интеграл простого отображения}

\begin{definition}
Пусть \(a_i\) - последовательность \(A\)\Hyph чисел.
Если
\ShowEq{sum |ai|<infty}
то мы будем говорить, что {\bf ряд}
\ShowEq{sum ai}
\AddIndex{сходится нормально}
{series converges normally}.\footnote{Смотри также
определение нормальной сходимости ряда
на странице \citeBib{Cartan differential form}-12.}
\qed
\end{definition}

\begin{definition}
\label{definition: integrable map}
Для простого отображения
\ShowEq{f:X->A}
рассмотрим ряд
\DrawEq{sum mu(F) f}{integral}
где
\begin{itemize}
\item
Множество
\ShowEq{f1...}
является областью определения отображения \(f\)
\item
Если \(n\ne m\), то
\ShowEq{fn ne fm}
\item
\DrawEq{Fn=}{-}
\end{itemize}
Простое отображение
\ShowEq{f:X->A}
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),
если ряд
\eqRef{sum mu(F) f}{integral}
сходится нормально.\footnote{Смотри
аналогичное определение в
\citeBib{Kolmogorov Fomin}, определение 2, с. 293.}
Если отображение \(f\) интегрируемо,
то сумма ряда
\eqRef{sum mu(F) f}{integral}
называется
\AddIndex{интегралом отображения}{integral of map}
\(f\) по множеству \(X\)
\ShowEq{integral of map}
\ShowEq{integral of simple map}
\qed
\end{definition}

\begin{theorem}
\label{theorem: integrable map}
Пусть
\ShowEq{f:X->A}
простое отображение.
Пусть \(f\) принимает значение\footnote{Мы не требуем
\ShowEq{fn ne fm}
при условии \(n\ne m\).
Однако мы требуем
\DrawEq{Fn Fm empty}{-}.
Смотри
также лемма в
\citeBib{Kolmogorov Fomin}, с. 293.} \(f_n\) на множестве
\ShowEq{Fn in X}
Пусть
\ShowEq{X=sum Fn}
\DrawEq{Fn Fm empty}{-}.
Отображение \(f\) интегрируемо тогда и только тогда, когда ряд
\DrawEq{sum mu(F) f}{int f}
сходится по норме. Тогда
\ShowEq{int f=sum mu(Fn)fn}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{Xi=}
Тогда
\ShowEq{Xi=sum Fn}
Из
\EqRef{Xi=sum Fn}
следует, что
\ShowEq{mu Xi=sum mu Fn}
Так как ряд
\eqRef{sum mu(F) f}{int f}
сходится по норме, то
\ShowEq{sum mu(Fn)fn 1}
следует из
\EqRef{mu Xi=sum mu Fn}.
\EqRef{int f=sum mu(Fn)fn}
следует из
\EqRef{integral of simple map},
\EqRef{sum mu(Fn)fn 1}.
\end{proof}

\begin{theorem}
\label{theorem: int f+g X simple}
Пусть
\ShowEq{f:X->A}
\ShowEq{g:X->A}
простые отображения.\footnote{Смотри
аналогичное утверждение в
\citeBib{Kolmogorov Fomin}, свойство А, с. 294.}
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{simple}
\end{theorem}
\begin{proof}
Пусть \(f\) принимает значение \(f_n\) на множестве
\ShowEq{Fn in X}
Пусть
\DrawEq{Fn Fm empty}{f+g}
Пусть \(g\) принимает значение \(g_k\) на множестве
\ShowEq{Gk in X}
Пусть
\DrawEq{Gk Gl empty}{f+g}
Равенство
\ShowEq{mu Fn=mu FnGk}
следует из равенства
\ShowEq{Fn=FnGk}
и условия
\eqRef{Gk Gl empty}{f+g}.
Равенство
\ShowEq{mu Gk=mu FnGk}
следует из равенства
\ShowEq{Gk=FnGk}
и условия
\eqRef{Fn Fm empty}{f+g}.
Условие
\ShowEq{FnGk FmGl empty}
следует из условий
\eqRef{Fn Fm empty}{f+g},
\eqRef{Gk Gl empty}{f+g}.

\StartLabelItem
\begin{enumerate}
\item
Так как отображение \(f\) интегрируемо, то равенство
\ShowEq{int f X=}
следует из
\EqRef{int f=sum mu(Fn)fn},
\EqRef{mu Fn=mu FnGk}
и ряд
\ShowEq{int f X=sum}
сходится по норме.
\LabelItem{int f X}
\item
Так как отображение \(g\) интегрируемо, то равенство
\ShowEq{int g X=}
следует из
\EqRef{int f=sum mu(Fn)fn},
\EqRef{mu Gk=mu FnGk}
и ряд
\ShowEq{int g X=sum}
сходится по норме.
\LabelItem{int g X}
\end{enumerate}
Из утверждений
\RefItem{int f X},
\RefItem{int g X}
следует, что
\ShowEq{int f+int g}
и ряд
\ShowEq{int f+g X=sum}
сходится по норме.
Следовательно, согласно теореме
\ref{theorem: integrable map},
равенство
\eqRef{int f+g X =}{simple}
следует из
\EqRef{int f+int g}.
\end{proof}

\begin{theorem}
\label{theorem: |int f|<int|f| simple}
Пусть
\ShowEq{f:X->A}
простое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{simple}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{sum|mu f|=sum mu|f|}
является следствием равенства
\ShowEq{|mu f|=mu|f|}
Следовательно, ряд
\DrawEq{sum mu(F) f}{}
сходится по норме тогда и только тогда, когда
сходится ряд
\ShowEq{sum mu(Fn)|fn|}
Неравенство
\eqRef{|int f|<int|f|}{simple}
следует из неравенства
\ShowEq{|sum|<sum||}
равенства
\EqRef{sum|mu f|=sum mu|f|}
и определения интеграла.
\end{proof}

\ifx\texFuture\Defined
\begin{theorem}
Пусть
\ShowEq{f12:X->R}
простые интегрируемые отображения такие, что
\ShowEq{f12>0}
почти всюду.
Отображение
\[h=f_1f_2\]
интегрируемо и
\ShowEq{int f12<int f1 int f2}
\end{theorem}
\begin{proof}
Если мы рассмотрим
\ShowEq{f 12 >0}
то неравенство
\ShowEq{f12<f 12}
очевидно.
Рассмотрим последовательности
\ShowEq{f12 n}
Пусть верно неравенство
\ShowEq{sum f12 m<sum f1m sum f2m}
Тогда неравенство
\ShowEq{sum f12 m+1}
следует из равенства
\EqRef{sum f12 m<sum f1m sum f2m}.
\end{proof}
\fi

\begin{theorem}
\label{theorem: |int omega f1n|<int|omega||f1n| simple}
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция в
абелевой \(\Omega\)\Hyph группе \(A\).
Пусть простое отображение
\ShowEq{fi:X->A}
интегрируемо. Тогда отображение
\DrawEq{h=f1...fn omega}{}
интегрируемо и
\DrawEq{|int h|<int|omega||f1n|}{}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: |int f|<int|f| simple}
и неравенства
\xEqRef{1305.4547}{|a omega|<|omega||a|1n}.
\end{proof}

\begin{theorem}
\label{theorem: A1->*A2 |int h|<int|g1||g2| simple}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{gi:X->A 12}
простое интегрируемое отображение.
Тогда отображение
\ShowEq{h=fX g1 g2}
интегрируемо и
\DrawEq{|int h|<int|g1||g2|}{}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: |int f|<int|f| simple}
и неравенства
\xEqRef{1305.4547}{|fab|<|f||a||b|}.
\end{proof}

\begin{theorem}
\label{theorem: int ag=a int g simple map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
эффективное представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть преобразования представления \(f\)
являются автоморфизмами представления
\EqParm{R->*Ak}{k=2}
Пусть
\ShowEq{g2:X->A2}
простое интегрируемое отображение
в нормированную $\Omega$\Hyph группу $A_2$.
Тогда отображение
\ShowEq{h=fX a1 g2}
интегрируемо и
\DrawEq{int ag=a int g}{simple}
\end{theorem}
\begin{proof}
Пусть \(g_2\) принимает значение \(g_{2\cdot k}\) на множестве
\ShowEq{Gk in X}
Пусть
\DrawEq{Gk Gl empty}{}
Так как отображение \(g_2\) интегрируемо, то равенство
\EquationParm{int gk X=}{k=2}
следует из
\EqRef{int f=sum mu(Fn)fn}
и ряд в
\EqRefParm{int gk X=}{k=2}
сходится по норме.
Согласно теореме
\xRef{1305.4547}{theorem: |fab|<|f||a||b|},
\ShowEq{|a1g2|<}
Следовательно, ряд
\ShowEq{mu a1g2}
сходится по норме.
Так как преобразование, порождённое \(a_1\in A_1\),
является автоморфизмом представления\footnote{Для нас здесь
важно, что для любых
\ShowEq{p a1 a2 b2}
Смотри также определение
\xRef{0912.3315}{definition: morphism of representations of F algebra}.
}
\EqParm{R->*Ak}{k=2}
равенство
\eqRef{int ag=a int g}{simple}
следует из равенства
\ShowEq{int ag=a int g 1}
и теоремы
\ref{theorem: integrable map}.
\end{proof}

\begin{theorem}
\label{theorem: int ga=int g a simple map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
эффективное представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть преобразования представления
\EqParm{R->*Ak}{k=1}
являются автоморфизмами представления \(f\).
Пусть
\ShowEq{g1:X->A1}
простое интегрируемое отображение
в нормированную $\Omega$\Hyph группу $A_1$.
Тогда отображение
\ShowEq{h=fX g1 a2}
интегрируемо и
\DrawEq{int ga=int g a}{simple}
\end{theorem}
\begin{proof}
Пусть \(g_1\) принимает значение \(g_{1\cdot k}\) на множестве
\ShowEq{Gk in X}
Пусть
\DrawEq{Gk Gl empty}{}
Так как отображение \(g_1\) интегрируемо, то равенство
\EquationParm{int gk X=}{k=1}
следует из
\EqRef{int f=sum mu(Fn)fn}
и ряд в
\EqRefParm{int gk X=}{k=1}
сходится по норме.
Согласно теореме
\xRef{1305.4547}{theorem: |fab|<|f||a||b|},
\ShowEq{|g1a2|<}
Следовательно, ряд
\ShowEq{mu g1a2}
сходится по норме.
Так как преобразование представления
\EqParm{R->*Ak}{k=1}
является автоморфизмом представления \(f\),
равенство\footnote{Для нас здесь
важно, что для любых
\ShowEq{p a1 b1 a2}
Смотри также определение
\xRef{0912.3315}{definition: morphism of representations of F algebra}.
}
\eqRef{int ga=int g a}{simple}
следует из равенства
\ShowEq{int ga=int g a 1}
и теоремы
\ref{theorem: integrable map}.
\end{proof}

\begin{theorem}
\label{theorem: int |f|<M mu simple map}
Пусть простое отображение
\ShowEq{f:X->A}
удовлетворяет условию
\DrawEq{|f(x)|<M}{int |f|}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{simple}
\end{theorem}
\begin{proof}
Пусть \(f\) принимает значение \(f_n\) на множестве
\ShowEq{Fn in X}
Пусть
\ShowEq{X=sum Fn}
\DrawEq{Fn Fm empty}{-}.
Согласно теореме
\ref{theorem: integrable map},
неравенство
\ShowEq{int |f|<M mu 1}
следует из равенства
\EqRef{int f=sum mu(Fn)fn}
и неравенства
\eqRef{|f(x)|<M}{int |f|}.
Неравенство
\eqRef{int |f|<M mu}{simple}
следует из неравенства
\EqRef{int |f|<M mu 1}.
\end{proof}

\begin{theorem}
\label{theorem: |int f|<M mu,  simple}
Пусть простое отображение
\ShowEq{f:X->A}
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
отображение \(f\) интегрируемо и
\DrawEq{|int f|<M mu}{simple}
\end{theorem}
\begin{proof}
Интегрируемость отображения \(f\) следует из теорем
\ref{theorem: |int f|<int|f| simple},
\ref{theorem: int |f|<M mu simple map}.
Неравенство
\eqRef{|int f|<M mu}{simple}
следует из неравенств
\eqRef{|int f|<int|f|}{simple},
\eqRef{int |f|<M mu}{simple}.
\end{proof}

\section{Интеграл измеримого отображения на множестве конечной меры}

\begin{definition}
\label{definition: Integral of Map over Set of Finite Measure}
\(\mu\)\Hyph измеримое отображение
\ShowEq{f:X->A}
называется
\AddIndex{интегрируемым}{integrable map}
по множеству \(X\),\footnote{Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 3, страницы 294, 295.
}
если существует последовательность
простых  отображений
\ShowEq{fn:X->A}
сходящаяся равномерно к \(f\).
Если отображение \(f\) интегрируемо,
то предел
\ShowEq{integral of map}
\ShowEq{integral of measurable map}
называется
\AddIndex{интегралом отображения}{integral of map}
\(f\) по множеству \(X\).
\qed
\end{definition}

\begin{theorem}
\label{theorem: Integral of Map over Set of Finite Measure}
Пусть
\ShowEq{f:X->A}
\(\mu\)\Hyph измеримое отображение.\footnote{Смотри также анализ определения
\citeBib{Kolmogorov Fomin}\Hyph 3, страница 295.
}
Пусть мера множества \(X\) конечна.
\StartLabelItem
\begin{enumerate}
\item
Для любой равномерно сходящейся последовательности
\(f_n\)
простых интегрируемых отображений
\ShowEq{fn:X->A}
предел
\EqRef{integral of measurable map}
существует.
\LabelItem{limit of integrals exists}
\item
Предел
\EqRef{integral of measurable map}
не зависит от выбора последовательности
\(f_n\).
\LabelItem{limit of integrals unique}
\item
Для простого отображения,
определение
\ref{definition: Integral of Map over Set of Finite Measure}
сводится к определению
\ref{definition: integrable map}.
\LabelItem{integral of simple map}
\end{enumerate}
\end{theorem}
\begin{proof}
Согласно теореме
\xRef{1305.4547}{theorem: sequence converges uniformly, fn-fm},
так как последовательность $f_n$ сходится равномерно
к отображению $f$,
то для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e/mu X}
для любых \(n\), \(m>N\).
Согласно теоремам
\ref{theorem: int f+g X simple},
\ref{theorem: |int f|<M mu,  simple},
\ShowEq{|int fm-int fn|}
следует из неравенства
\EqRef{|fn(x)-fm(x)|<e/mu X}
для любых \(n\), \(m>N\).
Согласно определению
\xRef{1305.4547}{definition: fundamental sequence}
и неравенству
\EqRef{|int fm-int fn|},
последовательность интегралов
\ShowEq{int mu fn}
является фундаментальной.
Следовательно, существует предел
\EqRef{integral of measurable map}
и утверждение
\RefItem{limit of integrals exists}
верно.

Пусть
\ShowEq{f12n}
- фундаментальные последовательности простых отображений,
равномерно сходящиеся к \(f\).
Согласно определению
\xRef{1305.4547}{definition: sequence converges uniformly},
так как последовательность \(f_{1\cdot n}\) сходится равномерно
к отображению $f$,
то для любого
\ShowEq{epsilon in R}
существует $N_1$ такое, что
\ShowEq{|f1n(x)-f(x)|<e/2mu X}
для любых
\ShowEq{n>N1}
Согласно определению
\xRef{1305.4547}{definition: sequence converges uniformly},
так как последовательность \(f_{2\cdot n}\) сходится равномерно
к отображению $f$,
то для любого
\ShowEq{epsilon in R}
существует $N_2$ такое, что
\ShowEq{|f2n(x)-f(x)|<e/2mu X}
для любых
\ShowEq{n>N2}
Пусть
\ShowEq{N N1 N2}
Из неравенств
\EqRef{|f1n(x)-f(x)|<e/2mu X},
\EqRef{|f2n(x)-f(x)|<e/2mu X}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|f1n(x)-f2n(x)|<e/mu X}
для любого $n>N$.
Согласно теоремам
\ref{theorem: int f+g X simple},
\ref{theorem: |int f|<M mu,  simple},
\ShowEq{|int f1n-int f2n|}
следует из неравенства
\EqRef{|f1n(x)-f2n(x)|<e/mu X}
для любого \(n>N\).
Согласно теореме
\xRef{1305.4547}{theorem: lim a=lim b}
и определению
\xRef{1305.4547}{definition: limit of sequence, Omega group},
\ShowEq{lim int f1n=lim int f2n}
следует из неравенства
\EqRef{|int f1n-int f2n|}
для любого \(n>N\).
Из равенства
\EqRef{lim int f1n=lim int f2n}
следует, что
утверждение
\RefItem{limit of integrals unique}
верно.

Пусть \(f\) - простое отображение.
Для доказательства справедливости утверждения
\RefItem{integral of simple map}
достаточно рассмотреть последовательность,
в которой \(f_n=f\) для любого \(n\).
\end{proof}

\begin{theorem}
\label{theorem: int f+g X}
Пусть
\ShowEq{f:X->A}
\ShowEq{g:X->A}
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Если существуют интегралы
\ShowEq{int f X}
\ShowEq{int g X}
то существует интеграл
\ShowEq{int f+g X}
и
\DrawEq{int f+g X =}{measurable}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
существует последовательность
простых  отображений
\ShowEq{fn:X->A}
сходящаяся равномерно к \(f\).
Согласно теореме
\ref{theorem: Integral of Map over Set of Finite Measure},
для любого
\ShowEq{epsilon in R}
существует \(N_1\) такое, что
\ShowEq{|int X f-fn|}
для любого
\ShowEq{n>N1}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
существует последовательность
простых  отображений
\ShowEq{gn:X->A}
сходящаяся равномерно к \(g\).
Согласно теореме
\ref{theorem: Integral of Map over Set of Finite Measure},
для любого
\ShowEq{epsilon in R}
существует \(N_2\) такое, что
\ShowEq{|int X g-gn|}
для любого
\ShowEq{n>N2}
Пусть
\ShowEq{N N1 N2}
Согласно теореме
\ref{theorem: int f+g X simple},
для любого
\(n>N\)
существует интеграл
\ShowEq{int X fn+gn}

Согласно теореме
\ref{theorem: f+g is measurable map},
отображение
\DrawEq{h=f+g}{int f+g X}
является $\mu$\Hyph измеримым отображением и
\ShowEq{h=lim fn+gn}

Если \(k\), \(n>N\), то
\ShowEq{int X f+g n-k}
следует из
\EqRef{|int X f-fn|},
\EqRef{|int X g-gn|},
\EqRef{int X fn+gn}.
Согласно определению
\xRef{1305.4547}{definition: fundamental sequence},
из неравенства
\EqRef{int X f+g n-k}
следует, что последовательность интегралов
\EqRef{int X fn+gn}
является фундаментальной.
Следовательно, согласно утверждениям
\eqRef{h=f+g}{int f+g X},
\EqRef{h=lim fn+gn}
и теореме
\ref{theorem: Integral of Map over Set of Finite Measure},
существует интеграл
\ShowEq{int X f+g=lim}

Если \(n>N\), то
\ShowEq{int X f+int X g n}
следует из
\EqRef{|int X f-fn|},
\EqRef{|int X g-gn|},
\EqRef{int X fn+gn}.
Из неравенства
\EqRef{int X f+int X g n}
следует, что последовательность интегралов
\EqRef{int X fn+gn}
является фундаментальной.
Согласно определению
\xRef{1305.4547}{definition: limit of sequence, Omega group},
\ShowEq{int X f+int X g=lim}

Равенство
\eqRef{int f+g X =}{measurable}
следует из равенств
\EqRef{int X f+g=lim},
\EqRef{int X f+int X g=lim}.
\end{proof}

\begin{theorem}
\label{theorem: |int f|<int|f|}
Пусть
\ShowEq{f:X->A}
измеримое отображение.
Интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Тогда
\DrawEq{|int f|<int|f|}{measurable}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: |int f|<int|f| simple}
и определения
\ref{definition: Integral of Map over Set of Finite Measure}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция в
абелевой \(\Omega\)\Hyph группе \(A\).
Пусть
\ShowEq{fi:X->A}
$\mu$\Hyph измеримое отображение
с компактным множеством значений.
Если отображение \(f_i\), \(i=1\), ..., \(n\),
интегрируемо, то отображение
\DrawEq{h=f1...fn omega}{}
интегрируемо и
\DrawEq{|int h|<int|omega||f1n|}{measurable}
\end{theorem}
\begin{proof}
Так как множество значений отображения
$f_i$
компактно,
то, согласно теореме
\xRef{1305.4547}{theorem: norm of compact set is bounded},
определена следующая величина
\DrawEq{F=sup|f|}{int|omega||f1n|}
Из равенства
\eqRef{F=sup|f|}{int|omega||f1n|}
и утверждения
\xRefItem{1305.4547}{|a|>=0}
следует, что
\DrawEq{F>0}{int|omega||f1n|}

Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
для \(i=1\), ..., \(n\), существует последовательность
простых  отображений
\ShowEq{fim:X->A}
сходящаяся равномерно к \(f_i\).
Из равенства
\DrawEq{fi(x)=lim}{}
и теоремы
\xRef{1305.4547}{theorem: sequence converges uniformly, fn-fm}
следует, что для заданного
\DrawEq{delta1 in R}{int|omega||f1n|}
существует $M_i$ такое, что из условия
\ShowEq{m>Mi}
следует
\ShowEq{|fim-fi|<d}
Пусть
\ShowEq{M M1 Mn}
Для \(k\), \(m>M\),
неравенство
\ShowEq{|fik-fim|<2d}
следует из неравенства
\EqRef{|fim-fi|<d}
и утверждения
\xRefItem{1305.4547}{|[a]+[b]|<=|[a]|+|[b]|}.
Для \(m>M\),
неравенство
\ShowEq{|fim|<Fi+d}
следует из
\xEqRef{1305.4547}{|a-b|>|a|-|b|},
\eqRef{F=sup|f|}{int|omega||f1n|},
\EqRef{|fim-fi|<d}
и неравенства
\ShowEq{|fim|<|fi|+d}

Согласно теореме
\ref{theorem: |int omega f1n|<int|omega||f1n| simple},
для любого
\(m>M\)
существует интеграл
\ShowEq{int X f1m...fnm omega}
Согласно утверждению
\xRefItem{1305.4547}{|a+b|<=|a|+|b|},
\ShowEq{int X f1n omega k-m 1}
Согласно определению
\xRef{1305.4547}{definition: Omega group},
\ShowEq{int X f1n omega k-m 2}
следует из
\eqRef{int f+g X =}{measurable},
\EqRef{int X f1n omega k-m 1}.
Согласно теореме
\ref{theorem: |int omega f1n|<int|omega||f1n| simple},
для любого
\(m>M\)
неравенство
\ShowEq{int X f1n omega k-m 3}
следует из неравенств
\EqRef{|fik-fim|<2d},
\EqRef{|fim|<Fi+d},
\EqRef{int X f1n omega k-m 2}.
Пусть
\ShowEq{e1=f(d1)}
Из утверждений
\eqRef{F>0}{int|omega||f1n|},
\eqRef{delta1 in R}{int|omega||f1n|}
следует, что
\DrawEq{e1>0}{int|omega||f1n|}
Из равенства
\EqRef{e1=f(d1)}
и утверждения
\eqRef{e1>0}{int|omega||f1n|}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\xRef{1305.4547}{theorem: image of interval is interval, real field},
отображение
\EqRef{e1=f(d1)}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\xRef{1305.4547}{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $M$ зависит от значения $\delta_1$.
Мы выберем значение $M$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $M$ такое, что из условия
$m>M$
следует
\ShowEq{int X f1n omega k-m}
Из равенства
\EqRef{int X f1n omega k-m}
следует, что последовательность интегралов
\EqRef{int X f1m...fnm omega}
является фундаментальной последовательностью.
Следовательность, последовательность интегралов
\EqRef{int X f1m...fnm omega}
имеет предел
\ShowEq{int X f1...fn omega=lim}

Согласно теореме
\ref{theorem: |int omega f1n|<int|omega||f1n| simple},
для любого
\(m>M\)
\ShowEq{|int f1m...fnm omega|<int |f1m|...|fnm| |omega|}
Неравенство
\eqRef{|int h|<int|omega||f1n|}{measurable}
следует из неравенства
\EqRef{|int f1m...fnm omega|<int |f1m|...|fnm| |omega|}
при предельном переходе
\ShowEq{m->infty}.
\end{proof}

\begin{theorem}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{gi:X->A 12}
интегрируемое отображение
с компактным множеством значений.
Тогда отображение
\ShowEq{h=fX g1 g2}
интегрируемо и
\DrawEq{|int h|<int|g1||g2|}{measurable}
\end{theorem}
\begin{proof}
Так как множество значений отображения
$g_i$
компактно,
то, согласно теореме
\xRef{1305.4547}{theorem: norm of compact set is bounded},
определена следующая величина
\ShowEq{G=sup|g|}
Из равенства
\EqRef{G=sup|g|}
и утверждения
\xRefItem{1305.4547}{|a|>=0}
следует, что
\ShowEq{G>0}

Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
для \(i=1\), \(2\), существует последовательность
простых  отображений
\ShowEq{gin:X->A}
сходящаяся равномерно к \(g_i\).
Из равенства
\ShowEq{gi(x)=lim}
и теоремы
\xRef{1305.4547}{theorem: sequence converges uniformly, fn-fm}
следует, что для заданного
\DrawEq{delta1 in R}{int|g1||g2|}
существует $N_i$ такое, что из условия
\ShowEq{n>Ni}
следует
\ShowEq{|gin-gi|<d}
Пусть
\ShowEq{N N1 N2}
Для \(k\), \(n>N\),
неравенство
\ShowEq{|gik-gin|<2d}
следует из неравенства
\EqRef{|gin-gi|<d}
и утверждения
\xRefItem{1305.4547}{|[a]+[b]|<=|[a]|+|[b]|}.
Для \(n>N\),
неравенство
\ShowEq{|gin|<Gi+d}
следует из
\xEqRef{1305.4547}{|a-b|>|a|-|b|},
\EqRef{G=sup|g|},
\EqRef{|gin-gi|<d}
и неравенства
\ShowEq{|gin|<|gi|+d}

Согласно теореме
\ref{theorem: A1->*A2 |int h|<int|g1||g2| simple},
для любого
\(n>N\)
существует интеграл
\ShowEq{int X fX g1n g2n}
Согласно утверждению
\xRefItem{1305.4547}{|a+b|<=|a|+|b|},
\ShowEq{int X fX g1 g2 k-m 1}
Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение \(f\) является гомоморфизмом абелевой группы \(A_1\)
и для любого \(a_1\in A_1\) отображение \(f(a_1)\)
является гомоморфизмом абелевой группы \(A_2\).
Следовательно,
\ShowEq{int X fX g1 g2 k-m 2}
следует из
\eqRef{int f+g X =}{measurable},
\EqRef{int X fX g1 g2 k-m 1}.
Согласно теореме
\ref{theorem: A1->*A2 |int h|<int|g1||g2| simple},
для любого
\(n>N\)
неравенство
\ShowEq{int X fX g1 g2 k-m 3}
следует из неравенств
\EqRef{|gik-gin|<2d},
\EqRef{|gin|<Gi+d},
\EqRef{int X fX g1 g2 k-m 2}.
Пусть
\ShowEq{e1=f(d1), fX g1 g2}
Из утверждений
\EqRef{G>0},
\eqRef{delta1 in R}{int|g1||g2|}
следует, что
\DrawEq{e1>0}{int|g1||g2|}
Из равенства
\EqRef{e1=f(d1), fX g1 g2}
и утверждения
\eqRef{e1>0}{int|g1||g2|}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\xRef{1305.4547}{theorem: image of interval is interval, real field},
отображение
\EqRef{e1=f(d1), fX g1 g2}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\xRef{1305.4547}{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $N$ зависит от значения $\delta_1$.
Мы выберем значение $N$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $N$ такое, что из условия
$n>N$
следует
\ShowEq{int X fX g1 g2 k-m}
Из равенства
\EqRef{int X fX g1 g2 k-m}
следует, что последовательность интегралов
\EqRef{int X fX g1n g2n}
является фундаментальной последовательностью.
Следовательность, последовательность интегралов
\EqRef{int X fX g1n g2n}
имеет предел
\ShowEq{int X fX g1 g2=lim}

Согласно теореме
\ref{theorem: A1->*A2 |int h|<int|g1||g2| simple},
для любого
\(n>N\)
\ShowEq{|int fX g1 g2|<int |g1n| |g2n| |f|}
Неравенство
\eqRef{|int h|<int|g1||g2|}{measurable}
следует из неравенства
\EqRef{|int fX g1 g2|<int |g1n| |g2n| |f|}
при предельном переходе
\ShowEq{n->infty}.
\end{proof}

\begin{theorem}
\label{theorem: int ag=a int g}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
эффективное представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть преобразования представления \(f\)
являются автоморфизмами представления
\EqParm{R->*Ak}{k=2}
Пусть
\ShowEq{g2:X->A2}
интегрируемое отображение
в нормированную $\Omega$\Hyph группу $A_2$.
Тогда отображение
\ShowEq{h=fX a1 g2}
интегрируемо и
\DrawEq{int ag=a int g}{}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: int ag=a int g simple map}
и определения
\ref{definition: Integral of Map over Set of Finite Measure}.
\end{proof}

\begin{theorem}
\label{theorem: int ga=int g a}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
эффективное представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть преобразования представления
\EqParm{R->*Ak}{k=1}
являются автоморфизмами представления \(f\).
Пусть
\ShowEq{g1:X->A1}
интегрируемое отображение
в нормированную $\Omega$\Hyph группу $A_1$.
Тогда отображение
\ShowEq{h=fX g1 a2}
интегрируемо и
\DrawEq{int ga=int g a}{}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: int ga=int g a simple map}
и определения
\ref{definition: Integral of Map over Set of Finite Measure}.
\end{proof}

\begin{theorem}
\label{theorem: int |f|<M mu}
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:X->A}
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
\DrawEq{int |f|<M mu}{measurable}
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: int |f|<M mu simple map}
и определения
\ref{definition: Integral of Map over Set of Finite Measure}.
\end{proof}

\begin{theorem}
\label{theorem: |int f|<M mu}
Пусть $\mu$\Hyph измеримое отображение
\ShowEq{f:X->A}
удовлетворяет условию
\DrawEq{|f(x)|<M}{}
Если мера множества \(X\) конечна, то
отображение \(f\) интегрируемо и
\DrawEq{|int f|<M mu}{measurable}
\end{theorem}
\begin{proof}
Интегрируемость отображения \(f\) следует из теорем
\ref{theorem: |int f|<int|f|},
\ref{theorem: int |f|<M mu}.
Неравенство
\eqRef{|int f|<M mu}{measurable}
следует из неравенств
\eqRef{|int f|<int|f|}{measurable},
\eqRef{int |f|<M mu}{measurable}.
\end{proof}

\section{Интеграл Лебега как отображение множества}
\label{section: Lebesgue Integral as Map of the Set}

Рассмотрим $\mu$\Hyph измеримое отображение
\ShowEq{f:X->A}
в $\Omega$\Hyph группу $A$.
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра измеримых множеств множества $X$.
Если
\ShowEq{Y in CX},
то мы можем рассматривать выражение
\ShowEq{Y->int Y f}
как отображение
\ShowEq{F:CX->A}

\begin{lemma}
\label{lemma: integral X=+Xi}
Пусть
\ShowEq{f:X->A}
простое отображение.
Пусть
\DrawEq{X=+Xi}{integral lemma}
конечное или счётное объединение множеств \(X_i\). 
Отображение \(f\) интегрируемо по множеству \(X\)
тогда и только тогда, когда
отображение \(f\) интегрируемо по каждому \(X_i\)
\DrawEq{integral X=+Xi}{lemma}
где ряд в правой части сходится по норме.
\end{lemma}
\begin{proof}
Пусть множество
\ShowEq{f1...}
является областью определения отображения \(f\).
Пусть
\DrawEq{Fn=}{X=+Xi}
\ShowEq{Fin=}
Равенства
\ShowEq{Fin=Fn*Xi}
\ShowEq{Fn=+Fin}
следуют из равенств
\eqRef{X=+Xi}{integral lemma},
\eqRef{Fn=}{X=+Xi},
\EqRef{Fin=}.
Равенство
\ShowEq{Fin*Fim}
следует из равенств
\eqRef{X=+Xi}{integral lemma},
\EqRef{Fin=Fn*Xi}.
Равенство
\ShowEq{mu(Fn=+Fin)}
следует из равенств
\EqRef{Fn=+Fin},
\EqRef{Fin*Fim}
и утверждения
\RefItem{mu(X=+Xi)}.
Равенство
\ShowEq{mu(Fn=+Fin)f}
следует из равенств
\eqRef{sum mu(F) f}{integral},
\EqRef{mu(Fn=+Fin)}.
Неравенство
\ShowEq{muFinf<muFnf<+muFinf}
следует из равенств
\EqRef{mu(Fn=+Fin)},
\EqRef{Fin=Fn*Xi}
и утверждения
\xRefItem{1305.4547}{|a+b|<=|a|+|b|}.
Неравенство
\ShowEq{+muFinf<+muFnf<++muFinf}
следует из неравенства
\EqRef{muFinf<muFnf<+muFinf}.
Сходимость по норме ряда
\ShowEq{++muFinf}
означает
\ShowEq{+n+i|muFinf|=+i+n|muFinf|}
\ShowEq{+n+imuFinf=+i+nmuFinf}
Из
\EqRef{+muFinf<+muFnf<++muFinf},
\EqRef{+n+i|muFinf|=+i+n|muFinf|}
следует, что ряд
\DrawEq{sum mu(F) f}{-}
сходится нормально
тогда и только тогда, когда
для любого \(i\)
ряд
\ShowEq{sum mu(Fin) f}
сходится нормально.
Согласно определению
\ref{definition: integrable map}
для каждого \(i\),
определён интеграл
\ShowEq{int Xi f}
Следовтельно, отображение \(f\) интегрируемо по множеству \(X\)
тогда и только тогда, когда
отображение \(f\) интегрируемо по каждому \(X_i\).
Равенство
\eqRef{integral X=+Xi}{lemma}
следует из равенств
\EqRef{mu(Fn=+Fin)f},
\EqRef{+n+imuFinf=+i+nmuFinf},
\EqRef{int Xi f}.
\end{proof}

\begin{theorem}[\(\sigma\)\Hyph аддитивность интеграла Лебега]
\label{theorem: integral X=+Xi}
Пусть
\ShowEq{f:X->A}
$\mu$\Hyph измеримое отображение.
Пусть
\DrawEq{X=+Xi}{integral}
конечное или счётное объединение множеств \(X_i\). 
Отображение \(f\) интегрируемо по множеству \(X\)
тогда и только тогда, когда
отображение \(f\) интегрируемо по каждому \(X_i\)
\DrawEq{integral X=+Xi}{theorem}
где ряд в правой части сходится по норме.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: Integral of Map over Set of Finite Measure},
для любого
\ShowEq{epsilon in R}
существует простое отображение
\ShowEq{g:X->A}
интегрируемое на \(X\) и такое, что для любого \(x\in X\)
\ShowEq{|f-g|<e}
Соглассно лемме
\ref{lemma: integral X=+Xi},
\ShowEq{integral X=+Xi g}
где \(g\) интегрируема на каждом \(X_i\)
и ряд
\EqRef{integral X=+Xi g}
сходится.
Согласно теореме
\ref{theorem: Integral of Map over Set of Finite Measure},
отображение \(f\) интегрируема на каждом \(X_i\).
Согласно теореме
\ref{theorem: |int f|<M mu},
\ShowEq{|int X f-g|}
\ShowEq{|int Xi f-g|}
следуют из
\EqRef{|f-g|<e}.
Согласно утверждениям
\xRefItem{1305.4547}{|a+b|<=|a|+|b|},
\RefItem{mu(X=+Xi)},
\ShowEq{sum|int Xi f-g|}
следует из
\eqRef{int f+g X =}{measurable},
\EqRef{|int Xi f-g|}.
Неравенство
\ShowEq{|int X f-sum int Xi f|}
следует из
\EqRef{|int X f-g|},
\EqRef{sum|int Xi f-g|}
и утверждения
\xRefItem{1305.4547}{|a|=0}.
Так как \(\epsilon\) произвольно,
то равенство
\eqRef{integral X=+Xi}{theorem}
следует из неравенства
\EqRef{|int X f-sum int Xi f|}.
\end{proof}

\begin{corollary}
Если $\mu$\Hyph измеримое отображение
\ShowEq{f:X->A}
интегрируемо на множестве \(X\),
то отображение \(f\) интегрируемо на $\mu$\Hyph измеримом множестве
\(X'\subset X\).
\qed
\end{corollary}

\begin{theorem}
\label{theorem: f(x)=g(x) almost everywhere, integral}
Пусть $\mu$\Hyph измеримые отображения
\ShowEq{f:X->A}
\ShowEq{g:X->A}
удовлетворяют условию
\DrawEq{|f(x)|<M}{f=g}
\ShowEq{|g(x)|<M}
Если
\(f(x)=g(x)\)
почти всюду, то
\ShowEq{int f(x)=int g(x)}
\end{theorem}
\begin{proof}
Из равенств
\eqRef{|f(x)|<M}{f=g},
\EqRef{|g(x)|<M}
и теоремы
\ref{theorem: |int f|<M mu}
следует, что
интегралы
\ShowEq{int f X}
\ShowEq{int g X}
существуют.
Пусть
\ShowEq{X1 f=g}
\ShowEq{X2 f ne g}
Так как
\ShowEq{X X1 X2}
то, согласно теореме
\ref{theorem: integral X=+Xi},
\ShowEq{int X=int X1+int X2, f}
\ShowEq{int X=int X1+int X2, g}
Согласно условию теоремы
\ShowEq{mu(X2)=0}
Из теоремы
\ref{theorem: |int f|<M mu},
утверждения
\xRef{1305.4547}{item: |a|>=0}
и равенства
\EqRef{mu(X2)=0}
следует, что
\ShowEq{int X2 f=0}
\ShowEq{int X2 g=0}
Равенство
\ShowEq{int X2 f=int X2 g=0}
следует из
\EqRef{int X2 f=0},
\EqRef{int X2 g=0}
и утверждения
\xRef{1305.4547}{item: |a|=0}.
Равенство
\ShowEq{int X1 f=int X1 g}
следует из
\EqRef{X1 f=g}.
Равенство
\EqRef{int f(x)=int g(x)}
следует из
\ShowEq{=>int f(x)=int g(x)}.
\end{proof}

\begin{theorem}[Неравенство Чебышева]
Если \(c>0\), то\footnote{Смотри также
\citeBib{Kolmogorov Fomin}, теорема на странице 300.
}
\ShowEq{mu(|f|>c)<int |f|/c}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{X'=(|f|>c)}
Тогда
\ShowEq{int X' f<c mu}
\EqRef{mu(|f|>c)<int |f|/c}
следует из
\EqRef{X'=(|f|>c)},
\EqRef{int X' f<c mu}.
\end{proof}

\begin{theorem}
\label{theorem: int|f|=0=>f=0}
Если
\ShowEq{int|f|=0}
то \(f(x)=0\) почти всюду.
\end{theorem}
\begin{proof}
Из
\EqRef{mu(|f|>c)<int |f|/c},
\EqRef{int|f|=0}
следует, что
\ShowEq{mu(f(x)>1/n)}
для \(n=1\), \(2\), ... .
Равенство
\ShowEq{mu(f=0)}
следует из
\EqRef{mu(f(x)>1/n)}.
\end{proof}

\begin{theorem}[Нормальная непрерывность интеграла Лебега]
\label{theorem: Normal continuity of Lebesgue integral}
Если\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 5, страницы 301, 302.
}
\ShowEq{f:X->A}
отображение, интегрируемое на множестве \(X\),
то для любого
\ShowEq{epsilon in R}
существует
\(\delta>0\)
такое, что
\ShowEq{|int E f(x)|}
для всякого
\ShowEq{E in CX}
такого, что
\ShowEq{mu(E)<d}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: |int f|<int|f|},
интеграл
\ShowEq{int f X}
существует
тогда и только тогда, когда
интеграл
\ShowEq{int |f| X}
существует.
Пусть
\ShowEq{Xi=(i<|f|<i+1)}
\ShowEq{YN=+Xi}
\ShowEq{ZN=X-YN}
Согласно теореме
\ref{theorem: integral X=+Xi},
\ShowEq{int X |f|=+int Xi |f|}
Так как ряд в
\EqRef{int X |f|=+int Xi |f|}
сходится по норме, то
существует \(N\) такое, что
\ShowEq{int ZN |f|<e/2}
Пусть
\ShowEq{d<e/2N}
Пусть
\ShowEq{mu(E)<d}
Тогда
\ShowEq{|int E f|<.+.}
Согласно теореме
\ref{theorem: int |f|<M mu},
неравенство
\ShowEq{int E*YN |f|}
следует из
\EqRef{Xi=(i<|f|<i+1)},
\EqRef{YN=+Xi}.
Неравенство
\ShowEq{int E*ZN |f|}
следует из
\EqRef{|int E f|<.+.}.
Неравенство
\EqRef{|int E f(x)|}
следует из неравенств
\EqRef{|int E f|<.+.},
\EqRef{int E*YN |f|},
\EqRef{int E*ZN |f|}.
\end{proof}

\section{Переход к пределу под знаком интеграла Лебега}

\begin{theorem}
\label{theorem: |f(x)|<g(x) is integrable}
Пусть отображение
\ShowEq{g:X->R}
интегрируемо и почти всюду
\DrawEq{|f(x)|<g(x)}{}
Тогда отображение \(f\) интегрируемо и
\ShowEq{|int f|<int g}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: f(x)=g(x) almost everywhere, integral},
\ShowEq{mu(X)=0=>int X f=0}
Следовательно, мы можем предположить,
что условие теоремы верно для любого \(x\in X\).
Теорема следует из теорем
\ref{theorem: |int f|<int|f|},
\citeBib{Kolmogorov Fomin}\Hyph \(VII\) на странице 297.
\end{proof}

\begin{theorem}[теорема Лебега о мажорируемой сходимости]
\label{theorem: Lebesgue's bounded convergence theorem}
Пусть\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 6 на страницах 302, 303.
}
\ShowEq{fn:X->A}
последовательность $\mu$\Hyph измеримых отображений
в $\Omega$\Hyph группу $A$ и
\DrawEq{f(x)=lim}{}
почти всюду.
Пусть отображение
\ShowEq{g:X->R}
интегрируемо и для всех \(n\in N\) почти всюду
\ShowEq{|fn(x)|<g(x)}
Тогда отображение \(f\) интегрируемо и
\DrawEq{int X f(x)=lim}{bounded convergence}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: f(x)=g(x) almost everywhere, integral},
\ShowEq{mu(X)=0=>int X f=0}
Следовательно, мы можем предположить,
что условие теоремы верно для любого \(x\in X\).
Согласно теореме
\citeBib{Fikhtengolts: Calculus volume 1}\Hyph 2 на странице 56,
неравенство
\DrawEq{|f(x)|<g(x)}{bounded convergence}
следует из неравенства
\EqRef{|fn(x)|<g(x)}.
Согласно теореме
\ref{theorem: |f(x)|<g(x) is integrable},
отображение \(f\) интегрируемо. 
Согласно теореме
\ref{theorem: Normal continuity of Lebesgue integral},
для любого
\ShowEq{epsilon in R}
существует
\(\delta>0\)
такое, что
\ShowEq{int Y g(x)<e/4}
для всякого
\ShowEq{Y in CX}
такого, что
\ShowEq{mu(Y)<d}
Согласно теореме
\ref{theorem: Egorov},
множество \(Y\),
удовлетворяющее условию
\EqRef{mu(Y)<d},
может быть выбрано таким образом, что
последовательность \(f_n\)
сходится равномерно на множестве
\ShowEq{Z=X-Y}
Согласно определению
\xRef{1305.4547}{definition: sequence converges uniformly},
найдётся \(N\) такое, что
при \(n>N\), \(x\in Z\) выполнено
\ShowEq{|fx-fnx|<e/2mu}
Неравенство
\ShowEq{|int f-fn|<e}
следует из равенства
\ShowEq{int Xf-int Xfn= YZ}
неравенств
\EqRef{|fn(x)|<g(x)},
\eqRef{|f(x)|<g(x)}{bounded convergence},
\EqRef{|fx-fnx|<e/2mu}
и теоремы
\ref{theorem: |int f|<M mu}.
Равенство
\eqRef{int X f(x)=lim}{bounded convergence}
является следствием неравенства
\EqRef{|int f-fn|<e}
и определения
\xRef{1305.4547}{definition: limit of sequence, Omega group}.
\end{proof}

\begin{corollary}
\label{corollary: int X f(x)=lim}
Если
\ShowEq{|fnx|<M}
и \(f_n\rightarrow f\), то
\DrawEq{int X f(x)=lim}{}
\qed
\end{corollary}

\begin{theorem}[Беппо Леви]
\label{theorem: Beppo Levi}
Пусть отображения\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 7 на странице 303.
}
\ShowEq{fn:A->R}
интегрируемы и
\ShowEq{int fn<M}
для некоторой константы \(M\).
Пусть для любого \(n\)
\ShowEq{fn(x)<fn1(x)}
Тогда почти всюду на \(A\) существует конечный предел
\ShowEq{f(x)=lim fn(x)}
Отображение \(f\) интегрируемо на \(A\) и
\ShowEq{int f=lim int fn}
\end{theorem}
\begin{proof}
Будем предполагать
\(f_1(x)\ge 0\),
так как в общем случае мы можем положить
\ShowEq{fi=fi-f1}
Согласно этому предположению и условию
\EqRef{fn(x)<fn1(x)}
\ShowEq{fn(x)>0}
Из утверждения
\EqRef{fn(x)>0}
и определений
\ref{definition: integrable map},
\ref{definition: Integral of Map over Set of Finite Measure}
следует, что для любого измеримого множества
\ShowEq{B in A}
\ShowEq{int B f>0}
Из теоремы
\ref{theorem: integral X=+Xi}
следует, что для любого измеримого множества
\ShowEq{B in A}
\ShowEq{int A f=int B f+}
Утверждение
\ShowEq{int B fn<M}
следует из
\EqRef{int fn<M},
\EqRef{int B f>0},
\EqRef{int A f=int B f+}.

Рассмотрим множество
\ShowEq{x in A f(x) infty}
Тогда
\ShowEq{Omega=*r+n}
где
\ShowEq{Omega nr=}
Согласно неравенству Чебышева
\EqRef{mu(|f|>c)<int |f|/c},
\ShowEq{Omega nr<}
следует из
\EqRef{int fn<M},
\EqRef{Omega nr=}.
Так как
\ShowEq{Omega nr in}
то
\ShowEq{+Omega nr<}
следует из
\EqRef{Omega nr<}.
Так как при любом \(r\)
\ShowEq{Omega in +Omega n}
то
\ShowEq{mu(Omega)<Mr}
Так как \(r\) произвольно, то
\ShowEq{mu(Omega)=0}
является следствием
\EqRef{mu(Omega)<Mr}.
Следовательно, монотонная последовательность
\(f_n(x)\)
почти всюду на \(A\) имеет конечный предел \(f(x)\).

Пусть
\ShowEq{Ar:r-1<f(x)<r}
\ShowEq{phi(x)=r}
Положим
\ShowEq{Bs=+Ar1s}
Из
\EqRef{Ar:r-1<f(x)<r},
\EqRef{Bs=+Ar1s}
следует, что
отображения \(f_n\) и \(f\) ограничены на \(B(s)\).
Из
\EqRef{Ar:r-1<f(x)<r},
\EqRef{phi(x)=r}
следует, что
\ShowEq{phi<f+1}
Согласно теоремам
\ref{theorem: A in B in Cmu=>mu A<mu B},
\ref{theorem: |f(x)|<g(x) is integrable},
\ShowEq{int phi<int f+mu}
следует из
\EqRef{phi<f+1}.
Согласно следствию
\ref{corollary: int X f(x)=lim},
\ShowEq{int phi<M+mu}
следует из
\EqRef{int B fn<M},
\EqRef{Ar:r-1<f(x)<r},
\EqRef{Bs=+Ar1s},
\EqRef{int phi<int f+mu}.
Согласно равенствам
\EqRef{Ar:r-1<f(x)<r},
\EqRef{phi(x)=r}
и определению
\ref{definition: simple map},
отображение \(\phi\) является простым.
Согласно определению
\ref{definition: integrable map},
\ShowEq{int Bs phi}
Сходимость ряда
\ShowEq{sum r mu Ar}
следует из
\EqRef{int phi<M+mu},
\EqRef{int Bs phi}.
Согласно определению
\ref{definition: simple map},
отображение \(\phi\) является интегрируемым
\ShowEq{int A phi}
Следовательно, утверждение теоремы является следствием теоремы
\ref{theorem: Lebesgue's bounded convergence theorem},
так как
\ShowEq{fn<f<phi}
следует из
\EqRef{fn(x)<fn1(x)},
\EqRef{int f=lim int fn},
\EqRef{Ar:r-1<f(x)<r},
\EqRef{phi(x)=r}.
\end{proof}





==> Measurable.Map.Russian.tex <==
%auto-ignore
\input{Measurable.Map.Eq}
\ifx\PrintBook\Defined
\chapter{Измеримое отображение в абелеву
\texorpdfstring{$\Omega$}{Omega}-группу}
\fi

\section{Измеримое отображение}

\begin{definition}
%\label{definition: }
Минимальная \(\sigma\)\Hyph алгебра
\ShowEq{Borel algebra}
над совокупностью всех открытых шаров нормированной $\Omega$\Hyph группы $A$,
называется
\AddIndex{алгеброй Бореля}{Borel algebra}.\footnote{Смотри
определение в
\citeBib{Kolmogorov Fomin}, с. 46.
Согласно замечанию
\ref{remark: A cup/minus B},
алгебра Бореля может быть также порождена множеством
замкнутых шаров.
}
Множество,
принадлежащее алгебре Бореля,
называется
\AddIndex{борелевским множеством}{Borel set}
или
\AddIndex{$B$\Hyph множеством}{B set}.
\qed
\end{definition}

\begin{definition}
\label{definition: C_X C_Y measurable}
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Отображение
\ShowEq{f:X->Y}
называется
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримым,\footnote{Смотри
аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282.}
если для всякого множества
\ShowEq{CX CY measurable map}
\qed
\end{definition}

\begin{example}
\label{example: measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{algebra of sets measurable with respect to measure}
- \(\sigma\)\Hyph алгебра измеримых относительно меры $\mu$ множеств.
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega$\Hyph группы $A$.
Отображение
\ShowEq{f:X->A}
называется
\AddIndex{$\mu$\Hyph измеримым}{mu measurable map},\footnote{Смотри
аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.
Если мера $\mu$ на множестве $X$ определена в контексте,
мы также будем называть отображение
\ShowEq{f:X->A}
\AddIndex{измеримым}{measurable map}.
}
если для всякого множества
\ShowEq{measurable map}
\qed
\end{example}

\begin{example}
Пусть
$\mathcal B(A)$
- алгебра Бореля
нормированной $\Omega_1$\Hyph группы $A$.
Пусть
$\mathcal B(B)$
- алгебра Бореля
нормированной $\Omega_2$\Hyph группы $B$.
Отображение
\ShowEq{f:A->B}
называется
\AddIndex{борелевским}{Borel-measurable map},\footnote{Смотри
аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 282, определение 1.}
если для всякого множества
\ShowEq{Borel-measurable map}
\qed
\end{example}

\begin{theorem}
\label{theorem: C_X C_Y C_Z measurable map}
Пусть $\mathcal C_X$ -
\(\sigma\)\Hyph алгебра множеств множества $X$.
Пусть $\mathcal C_Y$ -
\(\sigma\)\Hyph алгебра множеств множества $Y$.
Пусть $\mathcal C_Z$ -
\(\sigma\)\Hyph алгебра множеств множества $Z$.
\StartLabelItem
\begin{enumerate}
\item
\LabelItem{C_X C_Y measurable map}
Пусть отображение
\ShowEq{f:X->Y}
$(\mathcal C_X,\mathcal C_Y)$\Hyph измеримо.
\item
\LabelItem{C_Y C_Z measurable map}
Пусть отображение
\ShowEq{g:Y->Z}
$(\mathcal C_Y,\mathcal C_Z)$\Hyph измеримо.
\end{enumerate}
Тогда отображение
\ShowEq{g circ f}
$(\mathcal C_X,\mathcal C_Z)$\Hyph измеримо.\footnote{Смотри
аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страницы 282, 283, теорема 1.}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A in CZ}
Согласно определению
\ref{definition: C_X C_Y measurable}
и утверждению
\RefItem{C_Y C_Z measurable map},
\ShowEq{g A in CY}
Согласно определению
\ref{definition: C_X C_Y measurable}
и утверждению
\RefItem{C_X C_Y measurable map},
\ShowEq{gf A in CX}
Следовательно, отображение
\ShowEq{g circ f}
$(\mathcal C_X,\mathcal C_Z)$\Hyph измеримо.
\end{proof}

\section{Простое отображение}

\begin{definition}
\label{definition: simple map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Отображение
\ShowEq{f:X->A}
в нормированную $\Omega$\Hyph группу $A$ называется
\AddIndex{простым отображением}{simple map},
если это отображение $\mu$\Hyph измеримо и
принимает не более, чем счётное множество значений.
\qed
\end{definition}

\begin{theorem}
\label{theorem: measurable simple map}
Пусть отображение
\ShowEq{f:X->A}
принимает не более, чем счётное множество значений
\ShowEq{range f}
.
Отображение $f$ $\mu$\Hyph измеримо тогда и только тогда, когда
все множества
\ShowEq{f(x)=y}
$\mu$\Hyph измеримы.\footnote{Смотри
аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 1.}
\end{theorem}
\begin{proof}
Каждое множество $\{y_n\}$ является борелевским множеством.
Так как $A_n$ является прообразом множества $\{y_n\}$,
то $A_n$ является $\mu$\Hyph измеримым, если отображение $f$
является $\mu$\Hyph измеримым.
Следовательно, условие теоремы необходимо.

Пусть все множества $A_n$ $\mu$\Hyph измеримы.
Прообраз $f^{-1}(B)$ борелевского множества $B\subset A$
$\mu$\Hyph измерим,
так как он является объединением
\ShowEq{union An}
не более чем счётного множества $\mu$\Hyph измеримых множеств $A_n$.
Следовательно, отображение $f$ $\mu$\Hyph измеримо и
условие теоремы достаточно.
\end{proof}

\begin{theorem}
\label{theorem: simple f is measurable on +Xi}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{f:X->A}
простое отображения
в нормированную $\Omega$\Hyph группу $A$.
Пусть отображение \(f\) $\mu$\Hyph измеримо на множестве
\ShowEq{Xi 1...}
Тогда отображение \(f\) $\mu$\Hyph измеримо на множестве
\ShowEq{+Xi}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{range f}
- область значений отображения $f$.
Согласно теореме
\ref{theorem: measurable simple map},
множество
\ShowEq{Yik=}
$\mu$\Hyph измеримо.
Согласно определениям
\ref{definition: sigma algebra of sets},
\ref{definition: sigma-additive measure},
множество
\ShowEq{Yk=+Yik}
$\mu$\Hyph измеримо.
Согласно теореме
\ref{theorem: measurable simple map},
отображение \(f\) $\mu$\Hyph измеримо на множестве
\ShowEq{+Xi}
\end{proof}

\begin{theorem}
\label{theorem: h=f+g simple maps}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{f:X->A}
\ShowEq{g:X->A}
простые отображения
в нормированную $\Omega$\Hyph группу $A$.
Тогда отображение
\DrawEq{h=f+g}{}
является простым отображением.\footnote{Смотри
аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 283, теорема 3.}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: simple map},
простые отображения $f$ и $g$ имеют конечные или счётные
области значений.
Пусть
\ShowEq{range f}
- область значений отображения $f$.
Пусть
\ShowEq{range g}
- область значений отображения $g$.
Тогда область значений отображения $h$
состоит из значений
\ShowEq{c=y+z}
и является конечным или счётным множеством.
Для каждого $c_{ij}$ множество
\ShowEq{h(x)=c}
$\mu$\Hyph измеримо.
Следовательно, отображение $h$ является простым отображением.
\end{proof}

\begin{theorem}
\label{theorem: h=f omega simple maps}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Пусть
\ShowEq{fi:X->A}
простые отображения
в нормированную $\Omega$\Hyph группу $A$.
Тогда отображение
\ShowEq{h=f omega}
является простым отображением.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: simple map},
простые отображения
\ShowEq{fi 1n}
имеют конечные или счётные
области значений.
Пусть
\ShowEq{range fi}
- область значений отображения $f_i$.
Тогда область значений отображения $h$
состоит из значений
\ShowEq{y=y omega}
и является конечным или счётным множеством.
Для каждого
\ShowEq{yi 1n}
множество
\ShowEq{h(x)=y}
$\mu$\Hyph измеримо.
Следовательно, отображение $h$ является простым отображением.
\end{proof}

\begin{theorem}
\label{theorem: fX g1 g2 simple map}
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{gi:X->A 12}
простое отображение.
Тогда отображение
\ShowEq{h=fX g1 g2}
является простым отображением.
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: simple map},
простые отображения $g_1$ и $g_2$ имеют конечные или счётные
области значений.
Пусть
\ShowEq{range g1}
- область значений отображения $g_1$.
Пусть
\ShowEq{range g2}
- область значений отображения $g_2$.
Тогда область значений отображения $h$
состоит из значений
\ShowEq{c=f y1 y2}
и является конечным или счётным множеством.
Для каждого $c_{ij}$ множество
\ShowEq{h(x)=c f}
$\mu$\Hyph измеримо.
Следовательно, отображение $h$ является простым отображением.
\end{proof}

\section{Действия над измеримыми отображениями}

\begin{theorem}
\label{theorem: limit of sequence of measurable maps}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Пусть $\{f_n\}$ - последовательность
$\mu$\Hyph измеримых отображений
\ShowEq{fn:X->A}
Пусть
\ShowEq{f:X->A}
такое отображение, что
\DrawEq{f(x)=lim}{1}
для каждого $x$.
Тогда отображение $f$ является $\mu$\Hyph измеримым отображением.
\end{theorem}
\begin{proof}
Докажем следующее равенство
\ShowEq{f(x) in B(a,R)}

\begin{itemize}
\item
Пусть
\ShowEq{f(x) in B(a,R) 1}
Согласно определению
\xRef{1305.4547}{definition: closed ball}
\DrawEq{f(x) in B(a,R) 2}{1}
Из равенства
\eqRef{f(x)=lim}{1}
следует, что для любого $k$ существует такое $n$, что для $m>n$
\ShowEq{f(x)-fm(x)}
Из равенств
\eqRef{f(x) in B(a,R) 2}{1},
\EqRef{f(x)-fm(x)}
следует, что
\ShowEq{f(x) in B(a,R) 3}
Из определения
\xRef{1305.4547}{definition: open ball}
и равенства
\EqRef{f(x) in B(a,R) 3}
следует, что для любого $k$ существует такое $n$, что для $m>n$
\DrawEq{fm(x) in B(a,R)}{}
Следовательно, мы доказали, что
\ShowEq{f(x) in B(a,R) 4}
\item
Пусть
\ShowEq{f(x) in B(a,R) 5}
Тогда существуют $k$, $n$ такие,
что для $m>n$
\DrawEq{fm(x) in B(a,R)}{2}
Из определения
\xRef{1305.4547}{definition: open ball}
и равенства
\eqRef{fm(x) in B(a,R)}{2}
следует, что
\ShowEq{f(x) in B(a,R) 6}
Из теоремы
\citeBib{Fikhtengolts: Calculus volume 1}\Hyph 2,
страница 56,
равенства
\eqRef{f(x)=lim}{1}
и неравенства
\EqRef{f(x) in B(a,R) 6}
следует, что
\DrawEq{f(x) in B(a,R) 2}{2}
Из определения
\xRef{1305.4547}{definition: closed ball}
и неравенства
\eqRef{f(x) in B(a,R) 2}{2}
следует, что
\ShowEq{f(x) in B(a,R) 1}
Следовательно, мы доказали, что
\ShowEq{f(x) in B(a,R) 7}
\item
Равенство
\EqRef{f(x) in B(a,R)}
следует из равенств
\EqRef{f(x) in B(a,R) 4},
\EqRef{f(x) in B(a,R) 7}.
\end{itemize}

Если отображения $f_n$ измеримы, то, согласно примеру
\ref{example: measurable map},
множества
\ShowEq{f(x) in B(a,R) 8}
измеримы.
Так как совокупность измеримых множеств
является \(\sigma\)\Hyph алгеброй, то из равенства
\EqRef{f(x) in B(a,R)}
следует, что множество
\ShowEq{f(x) in B(a,R) 9}
измеримо.
Согласно примеру
\ref{example: measurable map},
отображение $f$ измеримо.
\end{proof}

\begin{theorem}
\label{theorem: uniformly convergent sequence of simple maps}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть множество значений отображения
\ShowEq{f:X->A}
компактно.
Отображение $f$ $\mu$\Hyph измеримо
тогда и только тогда, когда
оно может быть представлено как предел
равномерно сходящейся последовательности простых отображений.\footnote{Смотри
аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 292, теорема 2.}
\end{theorem}
\begin{proof}
Пусть отображение $f$ является пределом
равномерно сходящейся последовательности простых отображений.
Согласно определению
\ref{definition: simple map},
простое отображение $\mu$\Hyph измеримо.
Согласно теореме
\ref{theorem: limit of sequence of measurable maps},
предел последовательности простых отображений $\mu$\Hyph измерим.
Следовательно, отображение $f$ $\mu$\Hyph измеримо.

Пусть отображение $f$ $\mu$\Hyph измеримо.
Для заданного $n$,
рассмотрим множество открытых шаров
\ShowEq{set of open balls, f}
Множество $B_f$ является открытым покрытием
множества значений отображения $f$.
Следовательно, существует конечное множество
\ShowEq{B'f}
являющееся открытым покрытием
множества значений отображения $f$.
Для $x\in X$, выберем открытый шар
\ShowEq{B'f 1}
и мы положим
\ShowEq{fn(x)=}
Отображение $f_n$ - простое.
Из равенств
\EqRef{B'f 1},
\EqRef{fn(x)=}
и определения
\xRef{1305.4547}{definition: open ball}
следует, что
\ShowEq{fn(x)-f(x)}
Из равенства
\EqRef{fn(x)-f(x)}
следует, что последовательность простых отображений $f_n$
равномерно сходится к отображению $f$.
\end{proof}

\begin{theorem}
\label{theorem: f is measurable on +Xi}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть множество значений отображения
\ShowEq{f:X->A}
компактно.
Пусть отображение \(f\) $\mu$\Hyph измеримо на множестве
\ShowEq{Xi 1n}
Тогда отображение \(f\) $\mu$\Hyph измеримо на множестве
\ShowEq{+Xi}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
для каждого \(i\) существует последовательность простых отображений
\ShowEq{fik:X->A}
равномерно сходящейся к отображению \(f\) на множестве \(X_i\).
Для каждого \(k\),
рассмотрим отображение
\ShowEq{fk:+Xi->X}
определённое правилом
\ShowEq{x in Xi=>fk(x)=fik(x)}
Так как отображение \(f_k\)
принимает не более, чем счётное множество значений,
на множестве \(X_i\),
то отображение \(f_k\)
принимает не более, чем счётное множество значений,
на множестве
\ShowEq{+Xi}
Согласно теореме
\ref{theorem: simple f is measurable on +Xi},
отображение \(f_k\)
измеримо на множестве
\ShowEq{+Xi}

Так как последовательность отображений \(f_k\)
равномерно сходится к отображению \(f\) на множестве \(X_i\),
то, согласно определению
\xRef{1305.4547}{definition: sequence converges uniformly},
для заданного
\ShowEq{epsilon in R}
существует $K_i$ такое, что из условия
$k>K_i$
следует
\ShowEq{|fk(x)-f(x)|<e}
для любого $x\in X_i$.
Пусть
\ShowEq{K=max K1n}
Тогда для заданного
\ShowEq{epsilon in R}
из условия
$k>K$
следует
\ShowEq{|fk(x)-f(x)|<e}
для любого
\ShowEq{x in +Xi}
Согласно определению
\xRef{1305.4547}{definition: sequence converges uniformly},
последовательность отображений \(f_k\)
равномерно сходится к отображению \(f\) на множестве
\ShowEq{+Xi}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
отображение \(f\) $\mu$\Hyph измеримо на множестве
\ShowEq{+Xi}
\end{proof}

\begin{theorem}
\label{theorem: f+g is measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть $A$ - полная $\Omega$\Hyph группа.
Пусть
\ShowEq{f:X->A}
\ShowEq{g:X->A}
$\mu$\Hyph измеримые отображения
с компактным множеством значений.
Тогда отображение
\DrawEq{h=f+g}{measurable}
является $\mu$\Hyph измеримым отображением
с компактным множеством значений.\footnote{Смотри
аналогичную теорему в
\citeBib{Kolmogorov Fomin}, страница 283, теорема 3.}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
существует последовательность простых отображений $f_n$
равномерно сходящихся к отображению $f$
и существует последовательность простых отображений $g_n$
равномерно сходящихся к отображению $g$.
Для каждого $n$, отображение
\ShowEq{hn=fn+gn}
является простым отображением
согласно теореме
\ref{theorem: h=f+g simple maps}.
Согласно теореме
\xRef{1305.4547}{theorem: h=f+g, converges uniformly}
последовательность отображений $h_n$
равномерно сходится к отображению $h$.
Согласно теореме
\ref{theorem: limit of sequence of measurable maps},
отображению $h$ является $\mu$\Hyph измеримым отображением.

Рассмотри открытое покрытие \(O_h\)
множества значений отображения \(h\).
Согласно определению
\xRef{1305.4547}{definition: open set},
открытое покрытие \(O_h\)
содержит множество открытых шаров
\ShowEq{set of open balls, h}
Рассмотрим множество открытых шаров
\ShowEq{set of open balls, fx}
Множество $B_f$ является открытым покрытием
множества значений отображения $f$.
Следовательно, существует конечное множество
\ShowEq{B'f}
являющееся открытым покрытием
множества значений отображения $f$.
Положим
\ShowEq{If=}
Рассмотрим множество открытых шаров
\ShowEq{set of open balls, gx}
Множество $B_g$ является открытым покрытием
множества значений отображения $g$.
Следовательно, существует конечное множество
\ShowEq{B'g}
являющееся открытым покрытием
множества значений отображения $g$.
Положим
\ShowEq{Ig=}
Положим
\ShowEq{Ih=}
Для любого \(x\in X\),
существует \(x'\in I_h\) такой, что
\ShowEq{fg in Bo}
Согласно теореме
\xRef{1305.4547}{theorem: c1+c2 in B},
утверждение
\ShowEq{h in Bo}
следует из
\eqRef{h=f+g}{measurable},
\EqRef{fg in Bo}.
Следовательно, множество открытых шаров
\ShowEq{B'h}
является конечным открытым покрытием
множества значений отображения $h$.
Согласно определению
\xRef{1305.4547}{definition: compact set},
множество значений отображения $h$ компактно.
\end{proof}

\begin{theorem}
\label{theorem: f1...fn omega is measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Пусть
\ShowEq{fi:X->A}
$\mu$\Hyph измеримые отображения
в полную $\Omega$\Hyph группу $A$.
Тогда отображение
\DrawEq{h=f1...fn omega}{}
является $\mu$\Hyph измеримым отображением.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
существует последовательность простых отображений $f_{i\cdot m}$
равномерно сходящихся к отображению $f_i$.
Для каждого $m$, отображение
\ShowEq{hm=f1m...fnm omega}
является простым отображением
согласно теореме
\ref{theorem: h=f omega simple maps}.
Согласно теореме
\xRef{1305.4547}{theorem: h=f1...fn omega, converges uniformly}
последовательность отображений $h_n$
равномерно сходится к отображению $h$.
\end{proof}

\begin{theorem}
\label{theorem: fX g1 g2 is measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{gi:X->A 12}
$\mu$\Hyph измеримое отображение.
Тогда отображение
\ShowEq{h=fX g1 g2}
является $\mu$\Hyph измеримым отображением.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: uniformly convergent sequence of simple maps},
существует последовательность простых отображений $f_{i\cdot m}$
равномерно сходящихся к отображению $f_i$.
Для каждого $m$, отображение
\ShowEq{f(g1n)(g2n)}
является простым отображением
согласно теореме
\ref{theorem: fX g1 g2 simple map}.
Согласно теореме
\xRef{1305.4547}{theorem: fX(g1)(g2), converges uniformly}
последовательность отображений $h_n$
равномерно сходится к отображению $h$.
\end{proof}

\section{Сходимость почти всюду}

\begin{definition}
\label{definition: converges almost everywhere}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Последовательность\footnote{Смотри
так же определение
\citeBib{Kolmogorov Fomin}\Hyph 2 на странице 286.}
\ShowEq{fn:X->A}
$\mu$\Hyph измеримых отображений
в $\Omega$\Hyph группу $A$
\AddIndex{сходится почти всюду}{converges almost everywhere},
если
\DrawEq{f(x)=lim}{almost everywhere}
для почти всех \(x\in X\),
т. е. множество \(x\), в которых
\eqRef{f(x)=lim}{almost everywhere}
не выполняется, имеет меру нуль.
\qed
\end{definition}

\begin{theorem}
\label{theorem: limit almost everywhere is measurable map}
Пусть на множестве $X$ определена \(\sigma\)\Hyph аддитивная мера $\mu$.
Если последовательность
\ShowEq{fn:X->A}
$\mu$\Hyph измеримых отображений
в $\Omega$\Hyph группу $A$
сходится к отображению
\ShowEq{f:X->A}
почти всюду,
то отображение \(f\) также $\mu$\Hyph измеримо.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{x in X, lim fn=f}
Согласно определению
\ref{definition: converges almost everywhere},
\ShowEq{mu B = 0}

{\hangindent=1cm
\setlength{\parindent}{1.6cm}

\begin{lemma}
\label{lemma: map f is measurable on B}
Отображение \(f\) $\mu$\Hyph измеримо на множестве \(B\).
\end{lemma}

{\sc Доказательство.}
Утверждение является следствием определения
\ref{definition: C_X C_Y measurable}
и теоремы
\ref{theorem: A in B, mu B=0}.
\hfill\(\odot\)

\begin{lemma}
\label{lemma: map f is measurable on A}
Отображение \(f\) $\mu$\Hyph измеримо на множестве \(A\).
\end{lemma}

{\sc Доказательство.}
Согласно замечанию
\ref{remark: A cup/minus B},
множество \(A\) $\mu$\Hyph измеримо.
Согласно теореме
\ref{theorem: limit of sequence of measurable maps},
отображение \(f\) $\mu$\Hyph измеримо на множестве \(A\).
\hfill\(\odot\)

}%\hangindent

Из теоремы
\ref{theorem: f is measurable on +Xi}
и из лемм
\ref{lemma: map f is measurable on B},
\ref{lemma: map f is measurable on A}
следует, что
отображение $f$ $\mu$\Hyph измеримо.
\end{proof}

\begin{theorem}[Дмитрий Фёдорович Егоров]
\label{theorem: Egorov}
Пусть\footnote{Смотри
так же теорему
\citeBib{Kolmogorov Fomin}\Hyph 6 на странице 287.}
последовательность $\mu$\Hyph измеримых отображений
\ShowEq{fn:X->A}
сходится на измеримом множестве \(E\) почти всюду
к отображению \(f\).
Тогда, для любого \(\delta>0\),
существует измеримое множество
\ShowEq{Ed in E}
такое, что
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{mu Ed>mu E-d}
\item
Последовательность \(f_n\) равномерно сходится на множестве \(E_{\delta}\)\ .
\LabelItem{fn converges uniformly on the set Ed}
\end{enumerate}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: limit almost everywhere is measurable map},
отображение \(f\) $\mu$\Hyph измеримо на множестве \(E\).
Пусть
\ShowEq{Enm=*|fi-f|<1/m}
\ShowEq{Em=+Enm}
Утверждение
\ShowEq{E1m in E2m in...}
следует из
\EqRef{Enm=*|fi-f|<1/m}.
Из утверждений
\EqRef{Em=+Enm},
\EqRef{E1m in E2m in...}
и теоремы
\ref{theorem: Continuity of sigma-additive measure, subset}
следует, что
для любого \(m\) и для любого \(\delta>0\),
существует \(n_0(m)\) такое, что
\ShowEq{mu (Em-E0m)<d}
Положим
\ShowEq{Ed=*E0m}
Если
\ShowEq{x in Ed}
то, для любого \(m=1\), \(2\), ...
и для любого \(i>n_0(m)\),
неравенство
\ShowEq{|fi(x)-f(x)|<1/m}
следует из
\EqRef{Enm=*|fi-f|<1/m},
\EqRef{Ed=*E0m}.
Утверждение
\RefItem{fn converges uniformly on the set Ed}
следует из неравенства
\EqRef{|fi(x)-f(x)|<1/m}
и определения
\xRef{1305.4547}{definition: sequence converges uniformly}.

Если
\ShowEq{x in E-Em},
то, из
\EqRef{Enm=*|fi-f|<1/m},
\EqRef{Em=+Enm}
следует, что
существуют сколь угодно большие значения \(i\),
для которых
\ShowEq{|fi(x)-f(x)|>1/m}
Следовательно, последовательность \(f_n(x)\) в точке
\ShowEq{x in E-Em}
не сходится к \(f(x)\).
Так как \(f_n\) сходится к \(f\) почти всюду, то
из теоремы
\ref{theorem: A in B, mu B=0}
следует, что
\ShowEq{mu E-Em=0}
Неравенство
\ShowEq{mu (E-E0m)<d}
следует из
\EqRef{mu (Em-E0m)<d},
\EqRef{mu E-Em=0}.
Утверждение
\RefItem{mu Ed>mu E-d}
является следствием неравенства
\ShowEq{mu E-Ed<d}
которое следует из неравенства
\EqRef{mu (E-E0m)<d}.
\end{proof}




==> Measure.Russian.tex <==
%auto-ignore
\input{Measure.Eq}
\ifx\PrintBook\Defined
\chapter{Мера}
\fi

\section{Алгебра множеств}

\begin{definition}
\label{definition: semiring of sets}
Непустая система множеств $\mathcal S$ называется
\AddIndex{полукольцом множеств}{semiring of sets},\footnote{Смотри
так же определение
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 43.}
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{empty in S}
\item
Если
\ShowEq{A, B in S}
то
\ShowEq{AB in S}
\item
Если
\ShowEq{A, A1 in S},
то множество \(A\) может быть представлено в виде 
\DrawEq{A=+Ai}{def}
где
\ShowEq{Ai*Aj=0}
\LabelItem{A=+Ai}
\end{enumerate}
Представление
\eqRef{A=+Ai}{def}
множества \(A\) называется
\AddIndex{конечным разложением множества}{finite expansion of set}
\(A\).
\qed
\end{definition}

\begin{definition}
\label{definition: algebra of sets}
Непустая система множеств $\mathcal R$ называется
\AddIndex{кольцом множеств}{ring of sets},\footnote{Смотри
так же определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 41.}
если условие
\ShowEq{A, B in R}
влечёт
\ShowEq{A, B in R 1}
Множество
\ShowEq{E in R}
называется
\AddIndex{единицей кольца множеств}{unit of ring of sets},
если
\ShowEq{A cap E=A}
Кольцо множеств с единицей называется
\AddIndex{алгеброй множеств}{algebra of sets}.
\qed
\end{definition}

\begin{remark}
\label{remark: A cup/minus B}
Для любых
\ShowEq{A cup/minus B}
Следовательно, если
\ShowEq{A, B in R},
то
\ShowEq{A cup/minus B R}
\qed
\end{remark}

\begin{theorem}
Кольцо множеств \(\mathcal R\) является полукольцом.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A, A1 in R}.
Тогда
\ShowEq{A=A1+A2}
где
\ShowEq{A2=A-A1}
\end{proof}

\begin{theorem}
\label{theorem: intersection of rings is ring}
Пересечение
\ShowEq{R=*R}
любого множества
колец является
кольцом.\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 42.}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A, B in R}.
Тогда для любого \(i\),
\ShowEq{A, B in Ri}
Согласно определению
\ref{definition: algebra of sets},
для любого \(i\),
\ShowEq{A, B in Ri 1}
Следовательно,
\ShowEq{A, B in R 1}
Согласно определению
\ref{definition: algebra of sets},
множество \(\mathcal R\)
является кольцом множеств.
\end{proof}

\begin{theorem}
\label{theorem: ring of sets generated by system of sets}
Для любой непустой системы множеств \(\mathcal C\),
существует одно и только одно кольцо множеств\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 2 на странице 42.}
\ShowEq{ring R(C)},
содержащее \(\mathcal C\)
и содержащееся в любом кольце множеств \(\mathcal R\)
таком, что \(\mathcal C\subset\mathcal R\).
\end{theorem}
\begin{proof}
Пусть кольца множеств
\ShowEq{R1 ne R2}
удовлетворяют условию теоремы.
Согласно теореме
\ref{theorem: intersection of rings is ring},
множество
\ShowEq{R1*R2}
является кольцом множеств,
удовлетворяющим условию теоремы.
Следовательно, если кольцо множеств
\ShowEq{ring R(C)}
сущестаует,
то оно единственно.

Пусть
\DrawEq{R=+X in C}{}
Множество \(\mathcal B(R)\)
всех подмножеств множества \(R\)
является кольцом множеств и
\ShowEq{C in B(R)}
Пусть \(\Sigma\) - совокупность колец множеств \(\mathcal R\)
таких, что
\DrawEq{C in R in B(R)}{-}.
Тогда, согласно теореме
\ref{theorem: intersection of rings is ring},
множество
\ShowEq{+R in sigma}
является кольцом множеств, которое удовлетворяет теореме.
\end{proof}

\begin{theorem}
\label{theorem: ring of sets generated by system of sets with unit}
Пусть \(\mathcal C\) - непустая система множеств.
Пусть
\DrawEq{R=+X in C}{algebra}
Если
\ShowEq{R in C}
то кольцо множеств
\ShowEq{ring R(C)}
является алгеброй множеств.
\end{theorem}
\begin{proof}
Множество \(\mathcal B(R)\)
всех подмножеств множества \(R\)
является кольцом множеств и
\ShowEq{C in B(R)}
Пусть \(\Sigma\) - совокупность колец множеств \(\mathcal R\)
таких, что
\DrawEq{C in R in B(R)}{algebra}
Из
\EqRef{R in C},
\eqRef{C in R in B(R)}{algebra}
следует, что
\ShowEq{R in R}
для любого
\ShowEq{R in Sigma}
Тогда, согласно теореме
\ref{theorem: intersection of rings is ring},
множество
\ShowEq{+R in sigma}
является наименьшим кольцом множеств
таким, что
\ShowEq{R C in P}
Из
\eqRef{R=+X in C}{algebra}
следует, что
\ShowEq{R*A=A}
для любого множества
\ShowEq{A in P}
Согласно определению
\ref{definition: algebra of sets},
кольцо множеств \(\mathcal P\)
является алгеброй множеств.
\end{proof}

\begin{theorem}
\label{theorem: algebra of sets generated by system of sets}
Для любой непустой системы множеств \(\mathcal C\),
существует одна и только одна алгебра множеств
\ShowEq{ring A(C)},
содержащая \(\mathcal C\)
и содержащаяся в любой алгебре множеств \(\mathcal R\)
такой, что \(\mathcal C\subset\mathcal R\).
\end{theorem}
\begin{proof}
Пусть
\DrawEq{R=+X in C}{}
Теорема следует из теорем
\ref{theorem: ring of sets generated by system of sets},
\ref{theorem: ring of sets generated by system of sets with unit},
если мы положим
\ShowEq{A(C)=R(R,C)}
\end{proof}

\begin{lemma}
\label{lemma: exists finite expansion of set, 1}
Пусть\footnote{Леммы
\ref{lemma: exists finite expansion of set, 1},
\ref{lemma: exists finite expansion of set, 2}
и теорема
\ref{theorem: ring of sets generated by semiring}
аналогичны леммам 1, 2
и теореме 3,
\citeBib{Kolmogorov Fomin}, страницы 43, 45.
}
\(\mathcal S\)
- полукольцо.
Пусть \(A\),
\ShowEq{A1n in S},
\ShowEq{Ai*Aj=0}.
Тогда существует конечное разложение множества \(A\)
\ShowEq{A=+Ai1s}
\end{lemma}
\begin{proof}
Для \(n=1\)
лемма следует из утверждения
\RefItem{A=+Ai}.

Пусть лемма верна для \(n=m\).
Пусть множества
\ShowEq{A1m+1}
удовлетворяют условию леммы.
Согласно предположению
\ShowEq{A=A1mB1p}
где
\ShowEq{Bi in S}
\ShowEq{Ai*Aj=0},
\ShowEq{Ai*Bj=0}
\ShowEq{Bi*Bj=0}
Согласно утверждению
\RefItem{AB in S}
\DrawEq{Bi1=A*Bi}{1}
Согласно утверждению
\RefItem{A=+Ai}
\DrawEq{Bi=+Bi1r}{1}
Так как
\ShowEq{A in +B1r}
то
\ShowEq{A=A1mB1p 1}
является следствием
\EqRef{A=A1mB1p},
\eqRef{Bi1=A*Bi}{1},
\eqRef{Bi=+Bi1r}{1}.
Следовательно, лемма верна для \(n=m+1\).

Согласно математической индукции, лемма верна для любого \(n\).
\end{proof}

\begin{lemma}
\label{lemma: exists finite expansion of set, 2}
Для любой конечной системы множеств
\ShowEq{A1n in S}
существует конечная система множеств
\ShowEq{B1t in S}
такая, что
\ShowEq{Ai=+Bj}
где
\ShowEq{Mi in 1t}
\end{lemma}
\begin{proof}
Для \(n=1\)
лемма очевидна, так как достаточно положить
\ShowEq{B1=A1}

Пусть лемма верна для \(n=m\).
Рассмотрим систему множеств
\ShowEq{A1m+1}.
Пусть
\ShowEq{Bi in S}
- множества, удовлетворяющие условию леммы по отношению к
\(A_1\), ..., \(A_m\).
Согласно утверждению
\RefItem{AB in S}
\DrawEq{Bi1=A*Bi}{2}
Согласно утверждению
\RefItem{A=+Ai}
\DrawEq{Bi=+Bi1r}{2}
Разложение
\ShowEq{A=+Bs1+Bp}
следует из леммы
\ref{lemma: exists finite expansion of set, 1}.
Разложение
\ShowEq{Ai=++Bsj}
следует из равенств
\EqRef{Ai=+Bj},
\eqRef{Bi=+Bi1r}{2}.
Из равенств
\eqRef{Bi1=A*Bi}{2},
\EqRef{A=+Bs1+Bp}
следует, что
\ShowEq{Bi*Bp=0}
Следовательно, из равенства
\eqRef{Bi=+Bi1r}{2}
следует, что
\ShowEq{Bij*Bp=0}
Следовательно, множества
\ShowEq{Bij Bp}
удовлетворяют условиям леммы по отношению к
\ShowEq{A1m+1}.
Следовательно, лемма верна для \(n=m+1\).

Согласно математической индукции, лемма верна для любого \(n\).
\end{proof}

\begin{theorem}
\label{theorem: ring of sets generated by semiring}
Пусть \(\mathcal S\) - полукольцо множеств.
Система \(\mathcal R\) множеств \(A\),
которые имеют конечное разложение
\DrawEq{A=+Ai}{}
является
\AddIndex{кольцом множеств, порождённым полукольцом множеств}
{ring of sets generated by semiring}
\(\mathcal S\).
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A, B in R}
Тогда
\DrawEq{A=+Ai}{ring}
\ShowEq{B=+Bi}
Из
\eqRef{A=+Ai}{ring},
\EqRef{B=+Bi}
и утверждения
\RefItem{AB in S}
следует, что
\ShowEq{Cij=AiBj}
Согласно лемме
\ref{lemma: exists finite expansion of set, 1}
\ShowEq{Ai,Bj=Cij+}
Из
\EqRef{Ai,Bj=Cij+}
следует, что
\ShowEq{A*-B}
Следовательно, \(\mathcal R\) является кольцом  множеств.
\end{proof}

\begin{theorem}
\label{theorem: algebra of sets generated by semiring of sets}
Пусть полукольцо множеств \(\mathcal C\) содержит единицу.
Тогда кольцо  множеств
\ShowEq{ring R(C)}
является алгеброй множеств.
\end{theorem}
\begin{proof}
Теорема является следствием теорем
\ref{theorem: algebra of sets generated by system of sets},
\ref{theorem: ring of sets generated by semiring}.
\end{proof}

\begin{definition}
\label{definition: sigma algebra of sets}
Кольцо множеств $\mathcal R$ называется
\AddIndex{\(\sigma\)\Hyph кольцом множеств}{sigma ring of sets},\footnote{Смотри
аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 45, определение 3.}
если условие
\ShowEq{Ai in R}
влечёт
\ShowEq{Ai in R 1}
\(\sigma\)\Hyph Кольцо множеств с единицей называется
\AddIndex{\(\sigma\)\Hyph алгеброй множеств}{sigma algebra of sets}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: intersection of sigma rings is sigma ring}
Пересечение
\ShowEq{R=*R}
любого множества
\(\sigma\)\Hyph колец является
\(\sigma\)\Hyph кольцом.\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 42.}
\end{theorem}
\begin{proof}
Если
\ShowEq{Ai in R}.
то для любых \(i\), \(j\),
\ShowEq{Ai in Rj}
Следовательно,
для любого \(j\),
\ShowEq{+A in Rj}
Следовательно,
\ShowEq{+A in R}
Согласно определению
\ref{definition: sigma algebra of sets},
множество \(\mathcal R\)
является \(\sigma\)\Hyph кольцом множеств.
\end{proof}

\begin{theorem}
\label{theorem: sigma ring of sets generated by system of sets}
Для любой непустой системы множеств \(\mathcal C\),
существует одно и только одно \(\sigma\)\Hyph кольцо
множеств\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 2 на странице 42.}
\ShowEq{sigma ring R(C)},
содержащее \(\mathcal C\)
и содержащееся в любом \(\sigma\)\Hyph кольце множеств \(\mathcal R\)
таком, что \(\mathcal C\subset\mathcal R\).
\end{theorem}
\begin{proof}
Пусть \(\sigma\)\Hyph кольца множеств
\ShowEq{R1 ne R2}
удовлетворяют условию теоремы.
Согласно теореме
\ref{theorem: intersection of sigma rings is sigma ring},
множество
\ShowEq{R1*R2}
является \(\sigma\)\Hyph кольцом множеств,
удовлетворяющим условию теоремы.
Следовательно, если \(\sigma\)\Hyph кольцо множеств
\ShowEq{sigma ring R(C)}
сущестаует,
то оно единственно.

Пусть
\DrawEq{R=+X in C}{}
Множество \(\mathcal B(R)\)
всех подмножеств множества \(R\)
является \(\sigma\)\Hyph кольцом множеств и
\ShowEq{C in B(R)}
Пусть \(\Sigma\) - совокупность \(\sigma\)\Hyph колец множеств \(\mathcal R\)
таких, что
\DrawEq{C in R in B(R)}{-}.
Тогда, согласно теореме
\ref{theorem: intersection of rings is ring},
множество
\ShowEq{+R in sigma}
является \(\sigma\)\Hyph кольцом множеств, которое удовлетворяет теореме.
\end{proof}

\begin{theorem}
\label{theorem: sigma algebra of sets generated by system of sets}
Для любой непустой системы множеств \(\mathcal C\),
существует одна и только одна \(\sigma\)\Hyph алгебра множеств
\ShowEq{sigma ring A(C)},
содержащая \(\mathcal C\)
и содержащаяся в любой \(\sigma\)\Hyph алгебре множеств \(\mathcal R\)
такой, что \(\mathcal C\subset\mathcal R\).
\end{theorem}
\begin{proof}
Пусть
\DrawEq{R=+X in C}{}
Теорема следует из теорем
\ref{theorem: sigma ring of sets generated by system of sets},
\ref{theorem: ring of sets generated by system of sets with unit},
если мы положим
\ShowEq{sigma A(C)=R(R,C)}
\end{proof}

\section{Мера}

\begin{definition}
\label{definition: measure}
Пусть \(\mathcal C_m\) - полукольцо множеств.\footnote{Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 265.}
Отображение
\ShowEq{m:Cm->R}
называется
\AddIndex{мерой}{measure},
если
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{m(A)>0}
\item
Отображение \(m\) аддитивно.
Если множество
\ShowEq{A in Cm}
имеет конечное разлоение
\DrawEq{A=+Ai Cm}{}
где
\ShowEq{Ai*Aj=0},
то
\ShowEq{m A=+m Ai}
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
\label{theorem: m(empty)=0}
\ShowEq{m(empty)=0}
\end{theorem}
\begin{proof}
Так как
\ShowEq{empty+*=empty}
то теорема является следствием утверждений
\RefItem{empty in S},
\RefItem{m A=+m Ai}.
\end{proof}

\begin{definition}
\label{definition: extension of measure}
Мера \(\mu\) называется\footnote{Смотри также определение
\citeBib{Kolmogorov Fomin}\Hyph 2 на странице 266.}
\AddIndex{продолжением меры}{extension of measure} \(m\), если
\ShowEq{Cm in Cmu}
и
\ShowEq{m A=mu A}
\qed
\end{definition}

\begin{theorem}
\label{theorem: extension of measure}
Пусть\footnote{Смотри также теорему
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 266.}
\ShowEq{R(Cm)}
- кольцо множеств, порождённое полукольцом множеств
\(\mathcal C_m\).
Для меры \(m\), заданной на полукольце множеств
\(\mathcal C_m\),
существует одно и только одно продолжение \(\mu\),
заданное на кольце множеств
\ShowEq{R(Cm)}.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: ring of sets generated by semiring},
для каждого множества
\ShowEq{A in R(Cm)}
существует конечное разложение
\DrawEq{A=+Ai Cm}{extension of measure}
где
\ShowEq{Ai*Aj=0}.
Положим
\DrawEq{mu A=+m Ai}{extension of measure}

Если существует два конечных разложения
\ShowEq{A=+Ai=+Bj Cm}
Так как
\ShowEq{Ai*Bj in Cm}
согласно утверждению
\RefItem{AB in S},
то
\ShowEq{+Ai=+Bj}
следует из утверждения
\RefItem{m A=+m Ai}.
Следовательно, величина \(\mu(A)\),
определённая равенством
\eqRef{mu A=+m Ai}{extension of measure},
не зависит от выбора конечного разложения
\eqRef{A=+Ai Cm}{extension of measure}.

Следовательно, мы построили отображение
\ShowEq{mu:R(Cm)->R}
которое удовлетворяет определению
\ref{definition: measure}.

Для любого продолжения \(\mu'\) меры \(m\)
и для конечного разложения
\eqRef{A=+Ai Cm}{extension of measure},
из утверждения
\RefItem{m A=+m Ai}
и определения
\ref{definition: extension of measure}
следует, что
\ShowEq{+m' Ai=+m Ai}
Следовательно, мера \(\mu'\) совпадает с мерой \(\mu\),
определённой равенством
\eqRef{mu A=+m Ai}{extension of measure}.
\end{proof}

\begin{definition}
\label{definition: complete measure}
Мера \(\mu\) называется
\AddIndex{полной}{complete measure},
если из условий
\ShowEq{B in A, mu(A)=0}
следует,
что множество \(B\) измеримо.
\qed
\end{definition}

\begin{theorem}
\label{theorem: A in B in Cmu=>mu A<mu B}
Пусть на множестве $X$ определена мера $\mu$.
Пусть\footnote{Смотри
также теорему
\citeBib{Kolmogorov Fomin}\Hyph 2, с. 267.
}
\DrawEq{A in B in Cmu}{mu A<mu B}
Тогда
\DrawEq{mu A<mu B}{A in B}
\end{theorem}
\begin{proof}
Равенство
\ShowEq{B=A+(B-A)}
следует из утверждения
\eqRef{A in B in Cmu}{mu A<mu B}.
Согласно замечанию
\ref{remark: A cup/minus B},
из утверждения
\eqRef{A in B in Cmu}{mu A<mu B}
следует, что
\ShowEq{B-A in Cmu}
Равенство
\ShowEq{mu,B=A+(B-A)}
следует из равенства
\EqRef{B=A+(B-A)}.
Согласно утверждению
\RefItem{muX>0},
\ShowEq{mu B-A>0}
Утверждение
\eqRef{mu A<mu B}{A in B}
является следствием утверждений
\RefItem{mu(X=+Xi)},
\EqRef{mu,B=A+(B-A)}.
\end{proof}

\begin{theorem}
\label{theorem: A in +Ai in Cmu=>mu A<+mu Ai}
Пусть на множестве $X$ определена мера $\mu$.
Пусть
\ShowEq{A in Ai in Cmu}
где \(\{A_i\}\)
конечная или счётная система множеств.
Тогда
\DrawEq{mu A<mu B}{}
\end{theorem}
\begin{proof}
Мы докажем теорему для случая \(2\) множеств.
Общий случай легко доказать методом математической индукции.
Если
\ShowEq{A in A1+A2}
то теорема следует из теоремы
\ref{theorem: A in B in Cmu=>mu A<mu B},
утверждения
\ShowEq{mu(A+B)<mu(A)+mu(B)}
и утверждения
\RefItem{muX>0}.
\end{proof}

\begin{theorem}
\label{theorem: A in B, mu B=0}
Пусть на множестве $X$ определена
полная мера $\mu$.
Пусть
\DrawEq{A in B in Cmu}{}
Если
\ShowEq{mu B=0}
то
\ShowEq{mu A=0}
\end{theorem}
\begin{proof}
Теорема является следствием
определения
\ref{definition: complete measure}
и теоремы
\ref{theorem: A in B in Cmu=>mu A<mu B}.
\end{proof}

\begin{remark}
\label{remark: complete measure}
Мы будем полагать,
что рассматриваемая мера является полной мерой.
\qed
\end{remark}

\begin{definition}
\label{definition: sigma-additive measure}
Пусть $\mathcal C_{\mu}$ -
\(\sigma\)\Hyph алгебра множеств множества $F$.\footnote{Смотри
аналогичные определения в
\citeBib{Kolmogorov Fomin}, определение 1 на странице 265
и определение 3 на странице 268.}
Отображение
%\ShowEq{mu:CF->A}
%в нормированную $\Omega$\Hyph группу $A$ называется
\ShowEq{mu:Cmu->R}
в поле действительных чисел $R$ называется
\AddIndex{\(\sigma\)\Hyph аддитивной мерой}{sigma-additive measure},
если для любого множества
\ShowEq{X in Cmu}
выполнены следующие условия.
\StartLabelItem
\begin{enumerate}
\item
\ShowEq{muX>0}
\item
Пусть
\DrawEq{X=+Xi}{}
конечное или счётное объединение множеств
\ShowEq{Xn in Cmu}
Тогда
\DrawEqParm{mu(X=+Xi)}X{}
где ряд в правой части сходится абсолютно.
\LabelItem{mu(X=+Xi)}
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
Пусть \(m\) - \(\sigma\)\Hyph аддитивная мера,
определённая на полукольце множеств \(\mathcal C_m\).
Тогда продолжение \(\mu\) меры \(m\),
заданное на кольце множеств
\ShowEq{R(Cm)},
является \(\sigma\)\Hyph аддитивной мерой.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A,Bn in R(Cm)}
Пусть
\ShowEq{A=+Bn}
Согласно теореме
\ref{theorem: ring of sets generated by semiring},
существуют конечные разложения
\ShowEq{A=+Aj,B=+Bj}
где
\ShowEq{Ak*Al Bk*Bl}
Пусть
\ShowEq{C=A*B}
Очевидно, что множества \(C_{nil}\)
попарно не пересекаются и
\ShowEq{A=+C B=+C}
Из равенства
\EqRef{A=+C B=+C}
и утверждения
\RefItem{mu(X=+Xi)}
следует, что
\ShowEq{mA=+mC mB=+mC}
Из равенства
\EqRef{A=+Aj,B=+Bj}
и теоремы
\ref{theorem: extension of measure}
следует, что
\ShowEq{mA=+mAj mB=+mBi}
Равенство
\ShowEq{mA=+mBn}
является следствием
\EqRef{mA=+mC mB=+mC},
\EqRef{mA=+mAj mB=+mBi}.
\end{proof}

\begin{theorem}[Непрерывность \(\sigma\)\Hyph аддитивной меры]
\label{theorem: Continuity of sigma-additive measure, supset}
Пусть\footnote{Смотри
также теорему
\citeBib{Kolmogorov Fomin}\Hyph 9 на странице 261.
}
\ShowEq{A1 supset A2 ...}
последовательность $\mu$\Hyph измеримых множеств.
Тогда
\ShowEq{mu A=lim mu An}
где
\ShowEq{A=*An}
\end{theorem}
\begin{proof}
Мы рассмотрим случай
\ShowEq{A empty}
Общий случай сводится к этому заменой \(A_n\) на
\ShowEq{An-A}
Согласно утверждению
\EqRef{A1 supset A2 ...}
\ShowEq{An=An-+...}
Согласно утверждению
\RefItem{mu(X=+Xi)},
равенство
\ShowEq{mu An=+}
следует из
\EqRef{An=An-+...}.
Поскольку ряд
\EqRef{mu An=+}
для \(n=1\) сходится,
его остаток
\EqRef{mu An=+}
стремится к \(0\), когда \(n\rightarrow\infty\).
Следовательно,
\ShowEq{lim mu An=0}
\end{proof}

\begin{theorem}[Непрерывность \(\sigma\)\Hyph аддитивной меры]
\label{theorem: Continuity of sigma-additive measure, subset}
Пусть\footnote{Смотри
также следствие теоремы
\citeBib{Kolmogorov Fomin}\Hyph 9 на страницах 261, 262.
}
\ShowEq{A1 subset A2 ...}
последовательность $\mu$\Hyph измеримых множеств.
Тогда
\ShowEq{mu A=lim mu An}
где
\ShowEq{A=+An}
\end{theorem}
\begin{proof}
Теорема следует из теоремы
\ref{theorem: Continuity of sigma-additive measure, supset},
если мы рассмотрим множества
\ShowEq{X-An}
\end{proof}

\section{Лебегово продолжение меры}

\begin{definition}
\label{definition: outer measure}
Пусть \(m\) - \(\sigma\)\Hyph аддитивная мера
на полукольце \(\mathcal S\) с единицей \(E\).\footnote{Смотри
определение
\citeBib{Kolmogorov Fomin}\Hyph 1, страница 272.}
\AddIndex{Внешняя мера}{outer measure}
множества
\ShowEq{A in E}
определена равенством
\ShowEq{m*A=inf}
где точная верхняя грань берётся по всем покрытиям множества \(A\)
конечными или счётными системами множеств
\ShowEq{Bn in S}
\qed
\end{definition}

\begin{theorem}[счётная полуаддитивность]
\label{theorem: countable subadditivity}
Если\footnote{Смотри
также теоремы
\citeBib{Kolmogorov Fomin}\Hyph 3 на страницах 256, 257,
\citeBib{Kolmogorov Fomin}\Hyph 1 на странице 272.}
\ShowEq{A in +An}
где \(\{A_n\}\) - конечная или счётная система множеств, то
\ShowEq{mu*A<+mu*An}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: outer measure},
для каждого \(A_n\)
существует конечная или счётная система множеств
\ShowEq{Pnk}
такая, что
\ShowEq{An in +Pnk}
\ShowEq{+m(Pnk)<}
Из
\EqRef{A in +An},
\EqRef{An in +Pnk}
следует, что
\ShowEq{A in +Pnk}
Согласно утверждению
\EqRef{A in +Pnk}
и определению
\ref{definition: outer measure},
неравенство
\ShowEq{mu*A<+mP}
следует из неравенства
\EqRef{+m(Pnk)<}.
\EqRef{mu*A<+mu*An}
является следствием
\EqRef{mu*A<+mP},
так как \(\epsilon\) произвольно.
\end{proof}

\begin{theorem}
\label{theorem: |mu*A-mu*B|<}
Для любых множеств \(A\), \(B\),
\ShowEq{|mu*A-mu*B|<}
\end{theorem}
\begin{proof}
Если
\ShowEq{mu*A>mu*B}
то утверждение
\ShowEq{mu*A<mu*B}
является следствием утверждения
\ShowEq{A in B+AB}
и теоремы
\ref{theorem: countable subadditivity}.
Если
\ShowEq{mu*B>mu*A}
то утверждение
\ShowEq{mu*B<mu*A}
является следствием утверждения
\ShowEq{B in A+AB}
и теоремы
\ref{theorem: countable subadditivity}.
Утверждение
\EqRef{|mu*A-mu*B|<}
является следствием утверждений
\EqRef{mu*A<mu*B},
\EqRef{mu*B<mu*A}.
\end{proof}

\begin{definition}
\label{definition: Lebesgue measurable}
Множество \(A\) называется
\AddIndex{измеримым по Лебегу}{Lebesgue measurable},
для любого
\ShowEq{epsilon in R}
существует
\ShowEq{B in R(S)}
такое, что\footnote{Смотри
определение
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 272.}
\DrawEq{mu*(AB)<e}{}
\qed
\end{definition}

Пусть \(\mathcal C_{\mu}\) - система измеримых по Лебегу множеств.

\begin{theorem}
\label{theorem: E-A is Lebesgue measurable}
Пусть \(m\) - \(\sigma\)\Hyph аддитивная мера
на полукольце \(\mathcal S\) с единицей \(E\).\footnote{Смотри
также замечание в
\citeBib{Kolmogorov Fomin}
после определения 2 на странице 272.}
Если множество \(A\) измеримо по Лебегу,
то множество \(E\setminus A\) также измеримо по Лебегу.
\end{theorem}
\begin{proof}
Пусть \(A\) - множество, измеримое по Лебегу.
Согласно определению
\ref{definition: Lebesgue measurable},
для любого
\ShowEq{epsilon in R}
существует
\ShowEq{B in R(S)}
такое, что
\DrawEq{mu*(AB)<e}{E-A}
Согласно замечанию
\ref{remark: A cup/minus B},
\ShowEq{E-B in R(S)}
Утверждение
\ShowEq{mu*(E-A E-B)<e}
следует из утверждения
\eqRef{mu*(AB)<e}{E-A}
и равенства
\ShowEq{AB=E-A E-B}
\end{proof}

\begin{theorem}
\label{theorem: A1,A2 in M=>A1-A2 in M}
Пусть
\ShowEq{A12}
Тогда
\ShowEq{A=A1-A2}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: Lebesgue measurable},
для любого
\ShowEq{epsilon in R}
существуют
\ShowEq{B12 in R(S)}
такое, что
\DrawEq{mu*(AB12)<e/2}{A1-A2}
Согласно замечанию
\ref{remark: A cup/minus B},
\ShowEq{B1-B2 in R(S)}
Утверждение
\DrawEq{mu*(AB)<e}{}
следует из утверждения
\eqRef{mu*(AB12)<e/2}{A1-A2},
утверждения
\ShowEq{A1-A2 B1-B2=A B 12}
и теоремы
\ref{theorem: countable subadditivity}.
\end{proof}

\begin{theorem}
\label{theorem: A in R(S), mu*=mu}
Пусть \(m\) - \(\sigma\)\Hyph аддитивная мера
на полукольце \(\mathcal S\) с единицей \(E\).\footnote{Смотри
также замечания
в \citeBib{Kolmogorov Fomin} на страницах 256
и 272.}
Пусть \(\mu\) - продолжение меры \(m\)
на кольцо множеств
\ShowEq{R(S)}.
Любое множество
\ShowEq{A in R(S)}
измеримо по Лебегу и
\ShowEq{mu*=mu}
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A in R(S)}.
Согласно определению
\ref{definition: semiring of sets}
и теореме
\ref{theorem: ring of sets generated by semiring},
множество \(A\) может быть представлено в виде 
\DrawEq{A=+Ai}{}
где
\ShowEq{Ai*Aj=0}.
Согласно теореме
\ref{theorem: extension of measure},
\DrawEq{mu A=+m Ai}{Lebesgue}
Согласно определению
\ref{definition: outer measure},
так как множества \(A_i\) покрывают множество \(A\), то
\ShowEq{mu*<mu}
следует из
\eqRef{mu A=+m Ai}{Lebesgue}.

Пусть
\ShowEq{Q in S}
- конечная или счётная система множеств, покрывающих множество \(A\).
Согласно теоремам
\ref{theorem: extension of measure},
\ref{theorem: A in +Ai in Cmu=>mu A<+mu Ai},
\ShowEq{mu(A)<+m(Q)}
Согласно определению
\ref{definition: outer measure},
\ShowEq{mu<mu*}
следует из
\EqRef{mu(A)<+m(Q)}.

\EqRef{mu*=mu}
следует из
\EqRef{mu*<mu},
\EqRef{mu<mu*}.
\end{proof}

\begin{theorem}
\label{theorem: system of Lebesgue measurable sets is algebra}
Система \(\mathcal C_{\mu}\) измеримых по Лебегу множеств
является алгеброй множеств.
\end{theorem}
\begin{proof}
Из теоремы
\ref{theorem: A1,A2 in M=>A1-A2 in M},
определения
\ref{definition: algebra of sets}
и равенств
\ShowEq{A*+B -}
следует, что
\(\mathcal C_{\mu}\) является кольцом множеств.
Кольцо множеств \(\mathcal C_{\mu}\) является алгеброй множеств,
так как \(E\in\mathcal C_{\mu}\) является единицей
кольца множеств \(\mathcal C_{\mu}\).
\end{proof}

\begin{theorem}
\label{theorem: Lebesgue measure is additive}
Отображение \(\mu^*(A)\) аддитивно
на алгебре множеств \(\mathcal C_{\mu}\).\footnote{Смотри
также теоремы
\citeBib{Kolmogorov Fomin}\Hyph 6 на странице 258
и \citeBib{Kolmogorov Fomin}\Hyph 3 на странице 273.}
\end{theorem}
\begin{proof}
Для доказательства теоремы достаточно рассмотреть случай двух множеств.
Пусть
\ShowEq{A12}
Согласно определению
\ref{definition: Lebesgue measurable},
для любого
\ShowEq{epsilon in R}
существуют
\ShowEq{B12 in R(S)}
такое, что
\DrawEq{mu*(AB12)<e/2}{additive}
Положим
\ShowEq{A=+A12 B=+B12}
Согласно теореме
\ref{theorem: system of Lebesgue measurable sets is algebra},
\ShowEq{A in Cmu}
Так как
\ShowEq{A1*A2=0}
то
\ShowEq{*B12 in}
Утверждение
\ShowEq{mu(*B12)<e}
следует из утверждения
\EqRef{*B12 in}
и теорем
\ref{theorem: countable subadditivity},
\ref{theorem: A in R(S), mu*=mu}.
Утверждение
\ShowEq{|mu(B)-mu*A|<e 12}
следует из утверждения
\eqRef{mu*(AB12)<e/2}{additive}
и теорем
\ref{theorem: |mu*A-mu*B|<},
\ref{theorem: A in R(S), mu*=mu}.
Так как мера аддитивна на алгебре множеств
\ShowEq{R(S)},
то утверждение
\ShowEq{mu(B)>mu*A}
следует из утверждений
\EqRef{mu(*B12)<e},
\EqRef{|mu(B)-mu*A|<e 12}.
Утверждение
\ShowEq{mu*A>+mu*A}
следует из утверждения
\ShowEq{AB in +AB12}
Утверждение
\ShowEq{+mu*A>mu*A}
следует из утверждения
\EqRef{mu*A>+mu*A}
и теоремы
\ref{theorem: countable subadditivity}.
Так как \(\epsilon\) может быть выбрано произвольно малым, то
\ShowEq{mu*A=+mu*A}
следует из утверждения
\EqRef{+mu*A>mu*A}.
\end{proof}

\begin{definition}
Если множество \(A\) измеримо по Лебегу,\footnote{Смотри
определение
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 272.}
то величина
\ShowEq{mu=mu*}
называется
\AddIndex{мерой Лебега}{Lebesgue measure}.
Отображение \(\mu\), определённое на алгебре множеств \(\mathcal C_{\mu}\),
называется
\AddIndex{лебеговым продолжением меры}{Lebesgue extension of measure}
\(m\).
\qed
\end{definition}

\begin{theorem}
\label{theorem: algebra of Lebesgue measurable sets is sigma algebra}
Алгебра множеств \(\mathcal C_{\mu}\)
является \(\sigma\)\Hyph алгеброй\footnote{Смотри
также теоремы
\citeBib{Kolmogorov Fomin}\Hyph 7 на странице 259
и \citeBib{Kolmogorov Fomin}\Hyph 5 на страницах 273, 274.}
с единицей \(E\).
\end{theorem}
\begin{proof}
Пусть
\(A_1\), ...,
- счётная система множеств, измеримых по Лебегу.
Пусть
\ShowEq{A=+An 1...}
Положим
\ShowEq{A'n=An-}
Из
\EqRef{A=+An 1...},
\EqRef{A'n=An-}
следует, что
\ShowEq{A=+A'n 1...}
где
\ShowEq{A'i*A'j=0}
Согласно теореме
\ref{theorem: system of Lebesgue measurable sets is algebra},
определению
\ref{definition: algebra of sets}
и замечанию
\ref{remark: A cup/minus B},
все множества \(A'_n\) измеримы по Лебегу.
Согласно теореме
\ref{theorem: system of Lebesgue measurable sets is algebra}
и определению
\ref{definition: outer measure},
для любого \(n\)
\ShowEq{+mu(A)1n<mu*A}
Следовательно, ряд
\ShowEq{+mu(A)1...}
сходится.
Следовательно,
для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{+mu(A')<e/2}
Согласно теореме
\ref{theorem: system of Lebesgue measurable sets is algebra},
\ShowEq{+mu(A')1N in M}
Согласно определению
\ref{definition: Lebesgue measurable},
из утверждения
\EqRef{+mu(A')1N in M}
следует, что
существует
\ShowEq{B in R(S)}
такое, что
\ShowEq{mu*(CB)<e/2}
Так как
\ShowEq{AB in CB+}
то из
\EqRef{+mu(A')<e/2},
\EqRef{mu*(CB)<e/2}
и теоремы
\ref{theorem: countable subadditivity}
следует, что
\DrawEq{mu*(AB)<e}{}
Согласно определению
\ref{definition: Lebesgue measurable},
\ShowEq{A in Cmu}

Так как
\ShowEq{*A=-+-A}
то теорема является следствием теоремы
\ref{theorem: E-A is Lebesgue measurable}.
\end{proof}

\begin{theorem}
\label{theorem: Lebesgue measure is sigma additive}
Отображение \(\mu(A)\) \(\sigma\)\Hyph аддитивно\footnote{Смотри
также теорему
\citeBib{Kolmogorov Fomin}\Hyph 4 на странице 273.}
на алгебре множеств \(\mathcal C_{\mu}\).
\end{theorem}
\begin{proof}
Пусть
\ShowEq{A=+Ai in M}
где
\ShowEq{Ai*Aj=0}.
Согласно теореме
\ref{theorem: algebra of Lebesgue measurable sets is sigma algebra},
\ShowEq{A in Cmu}
Согласно теореме
\ref{theorem: countable subadditivity},
\ShowEq{mu(A)<+mu(Ai)}
Согласно теореме
\ref{theorem: Lebesgue measure is additive},
для любого \(N\)
\ShowEq{mu(A)>+mu(Ai) N}
и следовательно
\ShowEq{mu(A)>+mu(Ai)}
Равенство
\ShowEq{mu(A)=+mu(Ai)}
следует из
\EqRef{mu(A)<+mu(Ai)},
\EqRef{mu(A)>+mu(Ai)}.
\end{proof}

\begin{theorem}
\label{theorem: A in B, B_1 supseteq B_2, Bn1 subseteq Bn2}
Пусть\footnote{Смотри
также лемму в
\citeBib{Kolmogorov Fomin} на странице 315.}
\ShowEq{A in Cmu}
Тогда существует множество \(B\) такое, что
\DrawEq{A in B}{measure}
\DrawEq{muA=muB}{measure}
\DrawEq{B=*Bn}{measure}
\DrawEq{B_1 supseteq B_2}{measure}
\DrawEq{Bn=+Bnk}{measure}
\ShowEq{Bnk in S}
\DrawEq{muBnk<muA+}{measure}
\DrawEq{Bn1 subseteq Bn2}{measure}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: Lebesgue measurable}
и теореме
\ref{theorem: ring of sets generated by semiring},
для любого \(n\) существует множество \(C_n\) такое, что
\ShowEq{A in Cn}
\ShowEq{muCn<muA}
\ShowEq{Cn=+Dnr}
Положим
\ShowEq{Bn=*Ck}
Утверждение
\eqRef{B_1 supseteq B_2}{measure}
следует из
\EqRef{Bn=*Ck}.
Утверждение
\ShowEq{A in Bn}
следует из
\EqRef{A in Cn},
\EqRef{Bn=*Ck}.
Утверждение
\eqRef{A in B}{measure}
следует из
\eqRef{B=*Bn}{measure},
\EqRef{A in Bn}.
Из
\EqRef{Cn=+Dnr},
\EqRef{Bn=*Ck}
следует, что
\ShowEq{Bn=+dnr}
Пусть
\ShowEq{Bnk=+dnr}
Утверждение
\eqRef{Bn1 subseteq Bn2}{measure}
следует из
\EqRef{Bnk=+dnr}.
Утверждение
\eqRef{Bn=+Bnk}{measure}
следует из
\EqRef{Bn=+dnr},
\EqRef{Bnk=+dnr}.
Утверждение
\EqRef{Bnk in S}
следует из
\EqRef{Bn=+dnr},
\EqRef{Bnk=+dnr}
и теоремы
\ref{theorem: ring of sets generated by semiring}.

Из утверждения
\eqRef{A in B}{measure}
и теоремы
\ref{theorem: A in B in Cmu=>mu A<mu B}
следует, что
\ShowEq{muA<muB}
Из утверждений
\eqRef{B=*Bn}{measure},
\EqRef{muCn<muA},
\EqRef{Bn=*Ck}
и теоремы
\ref{theorem: A in B in Cmu=>mu A<mu B}
следует, что
\ShowEq{muB<muA+1n}
Так как \(n\) произвольно, то утверждение
\ShowEq{muB<muA}
является следствием утверждения
\EqRef{muB<muA+1n}.
Утверждение
\eqRef{muA=muB}{measure}
является следствием утверждений
\EqRef{muA<muB},
\EqRef{muB<muA}.
Утверждение
\eqRef{muBnk<muA+}{measure}
является следствием утверждений
\eqRef{Bn=+Bnk}{measure},
\EqRef{muB<muA+1n}
и теоремы
\ref{theorem: A in B in Cmu=>mu A<mu B}.
\end{proof}



==> Preface.1310.5591.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\ifx\PrintBook\Defined
\chapter{Preface}
\fi

\section{Preface to Version 1}

The theory of measurable functions and integral developed
in the middle of XX century solves a lot of mathematical problems.
However this theory considers real functions.

When I initiated study of algebra with continuous basis,
I realized that I need similar theory of integration
in normed vector space.
I considered integral of map into ring,
module and algebra. The common in these algebraic structures
is that they are Abelian group
with respect to addition. This property is enough to
study integration.

It was natural to consider the problem from the general point of view.
I recalled that some time ago I faced similar task.
So I decided to explore normed
$\Omega$\Hyph group and the theory of integration of 
maps into $\Omega$\Hyph group.

%We also
%assume that Abelian Group насследует norm of
%corresponding it algebra.

There are a lot of references to similar definitions
and theorems; so a reader sees that theory of integration
of maps into $\Omega$\Hyph group
has a lot of common with theory of integration
of functions of real variable.
However I had to change some statements,
since they implicitly assume either compactness of
range or total order
in $\Omega$\Hyph group.

I have devoted much attention to the topology
of normed $\Omega$\Hyph group.
To determine the integral of measurable map $f$,
I have to consider a sequence of
simple maps uniformly convergent
to the map $f$.

\begin{flushright}
October, 2013
\end{flushright}

\section{Preface to Version 2}

When I was writing the text of version 1,
I had to stop on Fubini's theorem.
The proof of the theorem depends significantly on
properties of real numbers.
This is not acceptable in the case of an arbitrary
\(\Omega\)\Hyph group.
However, we cannot extract matrix of linear transformation
of algebra with continuous basis
if we do not use Fubini's theorem.
So I returned to the paper
to prove Fubini's theorem.

The section
\ref{section: Lebesgue Integral as Map of the Set}
is very important now for me.
From theorems of the section
\ref{section: Lebesgue Integral as Map of the Set},
it follows that
properties of integral are similar to properties of measure.
It is attractive to consider more general definition of measure.
The text of paper is ready to generalization.
However the following problem should be resolved before.
Let \(\mu\) be measure with value in \(\Omega\)\Hyph group.
Let
\ShowEq{muA muB ne 0}
We require that
\ShowEq{mu A+B ne 0}
We can make this request as part of definition.

Since I consider integral of map into \(\Omega\)\Hyph group \(A\),
I had to define interaction
of real number and \(A\)\Hyph number.
I consider the representation of real field in
\(\Omega\)\Hyph group \(A\).
This consideration is essential
when I study algebra with continuous basis.

\begin{flushright}
March, 2014
\end{flushright}




==> Preface.1310.5591.Eq.tex <==
%auto-ignore

\DefEq
{
\(\mu(A)\ne 0\), \(\mu(B)\ne 0\).
}
{muA muB ne 0}

\DefEq
{
\(\mu(A\cup B)\ne\emptyset\).
}
{mu A+B ne 0}





==> Preface.1310.5591.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\ifx\PrintBook\Defined
\chapter{Предисловие}
\fi

\section{Предисловие к изданию 1}

Теория измеримых функций и интеграла, построенная
в середине XX века, решает немало математических проблем.
Однако эта теория рассматривает функции действительного переменного.

Когда я начал исследовать алгебры с непрерывным базисом,
я понял, что мне необходима аналогичная теория интегрирования
в нормированном векторном пространстве.
Я рассматривал интеграл отображений в кольца,
модули и алгебры. Эти алгебраические структуры
имеют то общее, что они являются абелевыми группами
относительно сложения. Этого свойства достаточно для
изучения операции интегрирования.

Естественно было рассмотреть проблему в общем,
и я вспомнил, что однажды такая задача передо мной стояла.
Так возникло решение изучить нормированные
$\Omega$\Hyph группы и теорию интегрирования
отображений в $\Omega$\Hyph группу.

%Мы также будем
%полагать, что абелева группа наследует норму
%соответствующей ей алгебры.

Из многочисленных ссылок на аналогичные определения
и теоремы, читатель увидит, что теория интегрирования
отображений в $\Omega$\Hyph группу
имеет много общего с теорией интегрирования
функций действительного переменного.
Однако многие утверждения необходимо изменить,
так как они неявно предполагают компактность
области значений либо отношение полного
порядка в $\Omega$\Hyph группе.

Я уделил большое внимание топологии
нормированной $\Omega$\Hyph группы.
Для определения интеграла измеримого отображения $f$,
мне надо рассмотреть последовательность
простых отображений, равномерно сходящихся
к отображению $f$.

\begin{flushright}
Октябрь, 2013
\end{flushright}

\section{Предисловие к изданию 2}

Когда я писал текст издания 1,
я был вынужден остановиться на теореме Фубини.
Доказательство теоремы существенно зависит
от свойств действительных чисел.
Это неприемлемо в случае произвольной
\(\Omega\)\Hyph группы.
Однако без теоремы Фубини невозможно
выделить матрицу линейного преобразования
алгебры с непрерывным базисом.
Поэтому я вернулся к статье
с целью доказать теорему Фубини.

Сейчас для меня
очень важен раздел
\ref{section: Lebesgue Integral as Map of the Set}.
Из теорем раздела
\ref{section: Lebesgue Integral as Map of the Set}
следует, что
свойства интеграла похожи на свойства меры.
Заманчиво рассмотреть более общее определение меры.
Текст статьи готов к обобщению.
Однако должна быть решена следующая задача.
Пусть \(\mu\) - мера со значением в \(\Omega\)\Hyph группе.
Пусть
\ShowEq{muA muB ne 0}
Мы требуем, чтобы
\ShowEq{mu A+B ne 0}
Это требование может быть частью определения меры.

Так как я рассматриваю интеграл отображения в \(\Omega\)\Hyph группу \(A\),
я должен был определить взаимодействие
действительного числа и \(A\)\Hyph числа.
Я рассматриваю представление поля действительных чисел в
\(\Omega\)\Hyph группу \(A\).
Эта модель удобна
при изучении алгебры с непрерывным базисом.

\begin{flushright}
Март, 2014
\end{flushright}



==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {единичный интервал}%
   {unit interval}%

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
\Symb%
   {минорная матрица}%
   {A without column a}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
\Symb%
   {минорная матрица}%
   {A without row b}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 1}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 2}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {CR linear combination in A module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левая дробь}%
   {left fraction}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
\Symb%
   {главный идеал}%
   {principal ideal}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {симплекс}%
   {simplex}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
\Symb%
   {замыкание множества}%
   {closure of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {открытый шар}%
   {open ball}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {правая дробь}%
   {right fraction}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
\Symb%
   {тензорное произведение представлений}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
\Symb%
   {структурные константы}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, scalar}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 1}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 2}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма функционала}%
   {norm of functional}%
\Symb%
   {норма отображения}%
   {norm of map}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
\Symb%
   {норма представления}%
   {norm of representation}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Symb%
   {сумма линейных отображений}%
   {sum of linear maps}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор отображения $f$}%
   {vector of mapping}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%
   {декартова степень систем подмножеств}%
   {Cartesian power of systems of subsets}%
\Symb%
   {декартово произведение систем подмножеств}%
   {Cartesian product of systems of subsets}%
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {множество \Acr линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
\Symb%
   {\rcd векторное пространство линейных отображений \drc векторного пространства $ V$ в \drc векторное пространство $W$}%
   {set linear maps, drc vector space}%
\Symb%
   {\drc векторное пространство линейных отображений \rcd векторного пространства $V$ в \rcd векторное пространство $W$}%
   {set linear maps, rcd vector space}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, scalar}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, vector}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований универсальной алгебры $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр отображения $f$}%
   {scalar of mapping}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {интеграл отображения \(f\)}%
   {integral of map}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%M%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Symb%
   {степень меры}%
   {power of measure}%
\Symb%
   {произведение мер}%
   {product of measures}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%

\SetIndexSpace%O%1
\Symb%
   {норма операции}%
   {norm of operation}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

